Modeling and Optimization Trade-off in Meta-learning

By searching for shared inductive biases across tasks, meta-learning promises to accelerate learning on novel tasks, but with the cost of solving a complex bilevel optimization problem. We introduce and rigorously define the trade-off between accurate modeling and optimization ease in meta-learning. At one end, classic meta-learning algorithms account for the structure of meta-learning but solve a complex optimization problem, while at the other end domain randomized search (otherwise known as joint training) ignores the structure of meta-learning and solves a single level optimization problem. Taking MAML as the representative meta-learning algorithm, we theoretically characterize the trade-off for general non-convex risk functions as well as linear regression, for which we are able to provide explicit bounds on the errors associated with modeling and optimization. We also empirically study this trade-off for meta-reinforcement learning benchmarks.

==> Neurips2020 (3)/math_header.tex <==
% This is roughly version 1.1 of vcl-shortcuts, circa Dec 2016.
% Put together by Vladlen Koltun

\usepackage{times}
\usepackage{epsfig}
\usepackage{graphicx}
\usepackage{float}
\usepackage{wrapfig}
\usepackage{amsmath,amssymb,amsthm}
\usepackage{algorithm,algorithmicx,algpseudocode}
\usepackage{bm,xspace}
\usepackage{comment}
\usepackage{verbatim}
\usepackage{multirow}
\usepackage{balance}
\usepackage{url}
\usepackage{booktabs}
\usepackage{etoolbox,siunitx}
\usepackage{calc}
\usepackage{pifont,hologo}
\usepackage[usenames, dvipsnames]{color}
\usepackage{nicefrac}

%Set up nice tables using the tabular package
%Make \toprule and \bottomrule thicker than \midrule
\setlength\heavyrulewidth{0.10em}
\setlength\lightrulewidth{0.05em}
\setlength\cmidrulewidth{0.03em}
\newcommand{\ra}[1]{\renewcommand{\arraystretch}{#1}}

%Set up the siunitx package, particularly for using the S column type in tables
\usepackage[super]{nth}
\usepackage{nicefrac}
\sisetup{detect-weight=true,detect-inline-weight=math}
\sisetup{quotient-mode = fraction}
\sisetup{fraction-function = \nicefrac}
\robustify\bfseries

% AMS stuff
\usepackage{dsfont}

\newtheorem{define}{Definition}
\newtheorem{theorem}{Theorem}
\newtheorem{lemma}{Lemma}
\newtheorem{cor}{Corollary}
\newtheorem{proposition}{Proposition}
\newtheorem{definition}{Definition}

\newcommand*{\eg}{e.g.\@\xspace}
\newcommand*{\ie}{i.e.\@\xspace}


%Known issue: the following shortcuts override \gg, \ll\, and \tt, which are existing LaTeX commands. Use \ggreater and \llesser, defined below, instead of \gg and \ll. Use \texttt{} instead of \tt.
%Also \ss is taken and in some environments cannot be overridden. Use \sss for a bold `s' instead.
\def\aa{\mathbf{a}}
\def\bb{\mathbf{b}}
\def\cc{\mathbf{c}}
\def\dd{\mathbf{d}}
\def\ee{\mathbf{e}}
\def\ff{\mathbf{f}}
\def\gg{\mathbf{g}}
\def\hh{\mathbf{h}}
\def\ii{\mathbf{i}}
\def\jj{\mathbf{j}}
\def\kk{\mathbf{k}}
\def\lll{\mathbf{l}}
\def\mm{\mathbf{m}}
\def\nn{\mathbf{n}}
\def\oo{\mathbf{o}}
\def\pp{\mathbf{p}}
\def\qq{\mathbf{q}}
\def\rr{\mathbf{r}}
\def\sss{\mathbf{s}}
\def\tt{\mathbf{t}}
\def\uu{\mathbf{u}}
\def\vv{\mathbf{v}}
\def\ww{\mathbf{w}}
\def\xx{\mathbf{x}}
\def\yy{\mathbf{y}}
\def\zz{\mathbf{z}}

\def\AA{\mathbf{A}}
\def\BB{\mathbf{B}}
\def\CC{\mathbf{C}}
\def\DD{\mathbf{D}}
\def\EE{\mathbf{E}}
\def\FF{\mathbf{F}}
\def\GG{\mathbf{G}}
\def\HH{\mathbf{H}}
\def\II{\mathbf{I}}
\def\JJ{\mathbf{J}}
\def\KK{\mathbf{K}}
\def\LL{\mathbf{L}}
\def\MM{\mathbf{M}}
\def\NN{\mathbf{N}}
\def\OO{\mathbf{O}}
\def\PP{\mathbf{P}}
\def\QQ{\mathbf{Q}}
\def\RR{\mathbf{R}}
\def\SSS{\mathbf{S}}
\def\TT{\mathbf{T}}
\def\UU{\mathbf{U}}
\def\VV{\mathbf{V}}
\def\WW{\mathbf{W}}
\def\XX{\mathbf{X}}
\def\YY{\mathbf{Y}}
\def\ZZ{\mathbf{Z}}

\def\aA{\mathcal{A}}
\def\bB{\mathcal{B}}
\def\cC{\mathcal{C}}
\def\dD{\mathcal{D}}
\def\eE{\mathcal{E}}
\def\fF{\mathcal{F}}
\def\gG{\mathcal{G}}
\def\hH{\mathcal{H}}
\def\iI{\mathcal{I}}
\def\jJ{\mathcal{J}}
\def\kK{\mathcal{K}}
\def\lL{\mathcal{L}}
\def\mM{\mathcal{M}}
\def\nN{\mathcal{N}}
\def\oO{\mathcal{O}}
\def\pP{\mathcal{P}}
\def\qQ{\mathcal{Q}}
\def\rR{\mathcal{R}}
\def\sS{\mathcal{S}}
\def\tT{\mathcal{T}}
\def\uU{\mathcal{U}}
\def\vV{\mathcal{V}}
\def\wW{\mathcal{W}}
\def\xX{\mathcal{X}}
\def\yY{\mathcal{Y}}
\def\zZ{\mathcal{Z}}

\def\Ae{\mathbb{A}}
\def\Be{\mathbb{B}}
\def\Ce{\mathbb{C}}
\def\Ee{\mathbb{E}}
\def\Le{\mathbb{L}}
\def\Ne{\mathbb{N}}
\def\Pe{\mathbb{P}}
\def\Qe{\mathbb{Q}}
\def\Re{\mathbb{R}}
\def\Se{\mathbb{S}}
\def\Te{\mathbb{T}}
\def\Xe{\mathbb{X}}
\def\Ye{\mathbb{Y}}
\def\Ze{\mathbb{Z}}

\def\btheta{{\bm\theta}}
\def\bzeta{{\bm\zeta}}
\def\bmu{{\bm\mu}}
\def\bZero{\mathbf{0}}
\def\bOne{\mathbf{1}}

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\minimize}{minimize}
\DeclareMathOperator*{\maximize}{minimize}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\rank}{rank}
\DeclareMathOperator{\trace}{tr}
\DeclareMathOperator{\diag}{diag}
\DeclareMathOperator{\diam}{diam}
\DeclareMathOperator{\var}{Var}

\def\eps{\varepsilon}
\def\vphi{\varphi}
\def\vsigma{\varsigma}

\def\trans{^{\intercal}}
\def\deg{^{\circ}}

\def\th{^{\textnormal{th}}}
\def\st{^{\textnormal{st}}}
\def\nd{^{\textnormal{nd}}}

%\ggreater and \llesser replace \gg and \ll, which have been overridden
\newcommand\ggreater{\mathbin{>\!\!\!>}}
\newcommand\llesser{\mathbin{<\!\!\!<}}

%Checkmark and cross symbols for tables
\newcommand{\YesV}{\ding{51}}%
\newcommand{\NoX}{\ding{55}}%

%Use @ instead of , in long numbers in math mode. For example, use $10@000$ rather than $10,000$.
\DeclareMathSymbol{@}{\mathord}{letters}{"3B}

\newcommand\paren[1]{\left(#1\right)}
\newcommand\abs[1]{\left\lvert#1\right\rvert}
\newcommand\norm[1]{\left\lVert#1\right\rVert}
\newcommand\tuple[1]{\left\langle#1\right\rangle}
\newcommand\inner[2]{\langle #1, #2 \rangle}

%Use \timess instead of \times in the main lines of equations, but not in superscripts or subscripts. Use the regular \times in superscripts or subscripts.
\newcommand\timess{\mathbin{\!\times\!}}

%Known issue: \nicebar is not nice in PNAS format, use \bar if submitting to PNAS.
\newcommand\nicebar[1]{\mkern 4mu\overline{\mkern-4mu#1}}

%Replace ``\yourname" and ``Name" with your name
\newcommand\ozan[1]{\textcolor{cyan}{Ozan says: #1}}
\newcommand\vladlen[1]{\textcolor{blue}{Vladlen says: #1}}
\newcommand\katelyn[1]{\textcolor{red}{Katelyn says: #1}}
\newcommand\creadych[1]{\textcolor{green}{Change in CR: #1}}
\newcommand\creadyadd[1]{\textcolor{cyan}{Add in CR: #1}}

%Paragraph heading with customizable vertical spacing. Modify the length inside \vspace to expand or contract the vertical offset preceding a new paragraph heading.
\newcommand\mypara[1]{\vspace{0mm}\noindent\textbf{#1}}

%Orient text vertically. Useful for tables and figures.
\def\rot#1{\rotatebox{90}{#1}}

%I use the self-indulgent \LaTeX operator mostly to illustrate an issue and a useful trick. The issue is that LaTeX operators eat the space that follows them, so if they occur in the middle of a sentence they eliminate the space separating the following word. But you can't just insert a space will-nilly (e.g., \LaTeX\ or \LaTeX~) because if the operator is followed by a punctuation mark then there shouldn't be a space. One solution is to write \LaTeX{}, which does the right thing but is easy to forget. The alternative, demonstrated here, is to define an operator with a name that ends with the forward slash. This also does the right thing and looks sufficiently distinctive to be memorable.
\def\latex/{\LaTeX}
\def\bibtex/{\hologo{BibTeX}}

%Miscellaneous \latex/ tips:
% To create an invisible character, use the \phantom command or its relatives: http://tex.stackexchange.com/questions/4519/how-do-i-create-an-invisible-character


==> Neurips2020 (3)/tex/complexity_proofs.tex <==
\subsection{Proof of Theorem~\ref{thm:drsamplecomplexity}}

\begin{proof}
We start with a generic bound on the gradient norm of a smooth function. Consider one step of SGD on a function $f(\cdot)$ that is $\mu$-smooth with learning rate $\beta^t$.

\begin{equation}
\begin{aligned}
    f(\btheta^{t+1}) &= f(\btheta^{t} - \beta^t\gg^t) \\
    &\leq f(\btheta^t) - \beta^t\nabla_{\btheta}f(\btheta^{t})^\intercal \gg^t + \frac{\mu {\beta^t}^2}{2}\|\gg^t\|^2_2 
\end{aligned}
\end{equation}
where $\gg^t$ is an estimate of the gradient of $f(\btheta^t)$.
Dividing by $\beta^t$ and moving the gradient term,
\begin{equation}
    \nabla_{\btheta}f(\btheta^t)^\intercal \gg^t \leq \frac{f(\btheta^t) - f(\btheta^{t+1})}{\beta^t} + \frac{\mu \beta^t}{2}\|\gg^t\|^2_2 
\end{equation}

During meta-training we take $T^{tr}$ steps of SGD on the loss $\rR^{drs}(\cdot)=\Ee_\gamma[\rR(\cdot;\gamma)]$ with learning rate $\beta^{tr}$ and during meta-testing we take $T^{te}$ steps of SGD on the task loss $\rR(\cdot;\gamma)$ with learning rate $\beta^{te}$.
Both losses are $\mu$-smooth by assumption.
Therefore, we can sum up the previous inequality over all $T$ steps, where $T=T^{tr}+T^{te}$.
\begin{equation}
\begin{aligned}
    &\sum_{t=0}^{T^{tr}-1} \nabla_{\btheta}\rR^{drs}(\btheta^t)^\intercal \gg^t+\sum_{t=T^{tr}}^{T-1} \nabla_{\btheta}\rR(\btheta^t;\gamma)^\intercal \gg^t \\
    &\leq \frac{\rR^{drs}(\btheta^0)-\rR^{drs}(\btheta^{T^{tr}})}{\beta^{tr}} + \frac{\rR(\btheta^{T^{tr}};\gamma)-\rR(\btheta^{T};\gamma)}{\beta^{te}} + \frac{\mu\beta^{tr}}{2}\sum_{t=0}^{T^{tr}-1}\|\gg^{t}\|_2^2 +
    \frac{\mu\beta^{te}}{2}\sum_{t=T^{tr}}^{T-1}\|\gg^{t}\|_2^2 \\
    &\leq \frac{\Delta}{\beta^{tr}} +  \frac{\rR(\btheta^{T^{tr}};\gamma) - \rR^{drs}(\btheta^{T^{tr}})}{\min\{\beta^{tr},\beta^{te}\}}  +
    \frac{ \rR(\btheta^*_{drs};\gamma) - \rR(\btheta^{T};\gamma)}{\beta^{te}} +
   \frac{\mu\beta^{tr}}{2}\sum_{t=0}^{T^{tr}-1}\|\gg^{t}\|_2^2 +
    \frac{\mu\beta^{te}}{2}\sum_{t=T^{tr}}^{T-1}\|\gg^{t}\|_2^2 \\
    &\leq \frac{\Delta}{\beta^{tr}} +  \frac{\rR(\btheta^{T^{tr}};\gamma) - \rR^{drs}(\btheta^{T^{tr}})}{\min\{\beta^{tr},\beta^{te}\}}  +
    \frac{ \rR(\btheta^*_{drs};\gamma)}{\beta^{te}} +
   \frac{\mu\beta^{tr}}{2}\sum_{t=0}^{T^{tr}-1}\|\gg^{t}\|_2^2 +
    \frac{\mu\beta^{te}}{2}\sum_{t=T^{tr}}^{T-1}\|\gg^{t}\|_2^2 \\
    &\leq \frac{\Delta +  \rR(\btheta^*_{drs};\gamma)}{\min\{\beta^{tr},\beta^{te}\}} +  \frac{\rR(\btheta^{T^{tr}};\gamma) - \rR^{drs}(\btheta^{T^{tr}})}{\min\{\beta^{tr},\beta^{te}\}}  +
   \frac{\mu\beta^{tr}}{2}\sum_{t=0}^{T^{tr}-1}\|\gg^{t}\|_2^2 +
    \frac{\mu\beta^{te}}{2}\sum_{t=T^{tr}}^{T-1}\|\gg^{t}\|_2^2 \\
    %&\leq \frac{\Delta}{\min\{\beta^{tr},\beta^{te}\}} + \frac{ \rR^{\star_{drs}}(\gamma) - \rR^{drs}(\btheta^{T};\gamma)}{\beta^{te}} +
   %\frac{\mu\beta^{tr}}{2}\sum_{t=0}^{T^{tr}-1}\|\gg^{t}\|_2^2 +
    %\frac{\mu\beta^{te}}{2}\sum_{t=T^{tr}}^{T-1}\|\gg^{t}\|_2^2 \\
    %&\leq \frac{\Delta+\Lambda^{drs}}{\min\{\beta^{tr},\beta^{te}\}} +\frac{\mu\beta^{tr}}{2}\sum_{t=0}^{T^{tr}-1}\|\gg^{t}\|_2^2 +
    %\frac{\mu\beta^{te}}{2}\sum_{t=T^{tr}}^{T-1}\|\gg^{t}\|_2^2.
\end{aligned}
\end{equation}

Recall that the task losses are $L$-Lipschitz.
For $t=0$ to $t=T^{tr}-1$,
\begin{align*}
    \gg^t &= \frac{1}{2NM}\sum_{j=1}^M\sum_{i=1}^{2N}\gg(\btheta^t,\xi_i;\gamma_j)\\
    \Ee(\gg^t) & = \Ee_\gamma[\nabla_\btheta\rR(\btheta^t;\gamma)]=\nabla_\btheta\rR^{drs}(\btheta^t) \\
    \Ee\norm{\gg^t}^2 &=\norm{\Ee(\gg^t)}^2+\trace(\var(\gg^t)) \leq L^2+V^t/M+V^d/2NM
\end{align*}
For $t=T^{tr}$ to $t=T-1$,
\begin{align*}
    \gg^t &= \frac{1}{N}\sum_{i=1}^{N}\gg(\btheta^t,\xi_i;\gamma)\\
    \Ee(\gg^t) &= \nabla_{\btheta}\rR(\btheta^t;\gamma) \\
    \Ee\norm{\gg^t}^2 &=\norm{\Ee(\gg^t)}^2+\trace(\var(\gg^t)) \leq L^2+V^d/N
\end{align*}

Therefore, taking expectation of both sides of the previous equation over $\gg^t$ and $\gamma$, and using the fact that $\Ee_{\gamma}[\rR(\btheta^{T^{tr}};\gamma)] = \rR^{drs}(\btheta^{T^{tr}})$ as well as $\Ee_{\gamma}[\rR(\btheta^*_{drs};\gamma)] = \Lambda^{drs}$,
\begin{equation}
\begin{aligned}
    &\sum_{t=0}^{T^{tr}-1} \norm{\nabla_{\btheta}\rR^{drs}(\btheta^t)}^2 + \sum_{t=0}^{T^{te}-1} \|\nabla_{\btheta}\rR(\btheta^{t+T^{tr}};\gamma)\|_2^2 \\
    &\leq \frac{\Delta + \Lambda^{drs}}{\min\{\beta^{tr},\beta^{te}\}} + \frac{\mu(\beta^{tr}T^{tr}(\frac{V^{d}}{2NM}+\frac{V^t}{M}+L^2)+\beta^{te}T^{te}(\frac{V^{d}}{N}+L^2))}{2} 
\end{aligned}
\end{equation}
We can further simplify the bound by assuming $\beta^{tr}=\beta^{te}$ and optimizing it over the learning rate.
Doing so, we obtain
\begin{equation}
\begin{aligned}
    \sum_{t=0}^{T^{tr}-1} \norm{\nabla_\btheta \rR^{drs}(\btheta^t)}^2 + \sum_{t=0}^{T^{te}-1} \|\nabla_{\btheta}\rR(\btheta^{t+T^{tr}};\gamma)\|^2  \leq  \sqrt{0.5\big(\Delta + \Lambda^{drs}\big) \big(C^{drs}_{tr}T^{tr} + C^{drs}_{te}T^{te}\big)}
\end{aligned}
\end{equation}
where
\begin{equation}
    C^{drs}_{tr}= 
    \mu\left(L^2+\frac{V^t}{M}+\frac{V^d}{2NM}\right) \text{ and }
C^{drs}_{te}= \mu\left(L^2+\frac{V^d}{N}\right) 
\end{equation}
\end{proof}

\subsection{Proof of Theorem~\ref{thm:mamlsamplecomplexity}}

\begin{proof}

From Corollary A.1 of \citet{mamlconvergence}, $\rR^{maml}(\btheta)$ has smoothness constant $\mu^{\prime} = 4\mu+2\mu^{H}\alpha L$. Thus, using a similar argument as in the proof of Theorem~\ref{thm:drsamplecomplexity},
\begin{equation}\label{eq:mamltraintest}
\begin{aligned}
    &\sum_{t=0}^{T^{tr}-1} \nabla_\btheta \rR^{maml}(\btheta^t;\alpha)^\intercal \gg^t+\sum_{t=T^{tr}}^{T-1} \nabla_{\btheta}\rR(\btheta^t;\gamma)^\intercal \gg^t \\
    &\leq \frac{\rR^{maml}(\btheta^0;\alpha)-\rR^{maml}(\btheta^{T^{tr}};\alpha)}{\beta^{tr}} + \frac{\rR(\btheta^{T^{tr}};\gamma)-\rR(\btheta^{T};\gamma)}{\beta^{te}} + \frac{\mu^\prime\beta^{tr}}{2}\sum_{t=0}^{T^{tr}-1}\|\gg^{t}\|_2^2 +
    \frac{\mu\beta^{te}}{2}\sum_{t=T^{tr}}^{T-1}\|\gg^{t}\|_2^2 \\
    &\leq \frac{\Delta +  \rR(\mamlsol-\alpha\nabla_\btheta\rR(\mamlsol;\gamma);\gamma)}{\min\{\beta^{tr},\beta^{te}\}} +  \frac{\rR(\btheta^{T^{tr}};\gamma) - \rR^{maml}(\btheta^{T^{tr}};\alpha)}{\min\{\beta^{tr},\beta^{te}\}}  \\
    &\quad+
   \frac{\mu^\prime\beta^{tr}}{2}\sum_{t=0}^{T^{tr}-1}\|\gg^{t}\|_2^2 +
    \frac{\mu\beta^{te}}{2}\sum_{t=T^{tr}}^{T-1}\|\gg^{t}\|_2^2 
\end{aligned}
\end{equation}
For $t=0$ to $t=T^{tr}-1$, using results from the proof of Theorem 5.12 in \citet{mamlconvergence},
\begin{align*}
    \gg^t &= \dfrac{1}{M}\sum_{j=1}^M \gg_j^t, \quad \gg_j^t=(I-\dfrac{\alpha}{D}\sum_{d=1}^D\hh(\btheta^t,\xi_d;\gamma_j))\sum_{i=1}^N\gg(\btheta^t-\dfrac{\alpha}{N}\sum_{j=1}^N\gg(\btheta^t,\xi_j;\gamma_j),\xi_i;\gamma_j)\\
    \Ee(\gg^t) &= \Ee(\gg_j^t) = \nabla_\btheta \rR^{maml}(\btheta^t;\alpha)+r^t
\end{align*}
where
\begin{align*}
    \norm{r^t} &\leq (1+\alpha\mu)\alpha\mu\sqrt{V^d/N} \\
    \norm{\nabla_\btheta \rR^{maml}(\btheta^t;\alpha)} &\leq \norm{\Ee_\gamma[(I-\alpha\nabla_\btheta^2\rR(\btheta^t;\gamma))\nabla_\btheta\rR(\btheta^t-\alpha\nabla_\btheta\rR(\btheta^t;\gamma);\gamma)]} \leq (1+\alpha\mu)L
\end{align*}
Define $\rho \triangleq (1+\alpha\mu)$. Then,
\begin{align*}
    \Ee\norm{\gg^t}^2 &\leq \norm{\Ee(\gg_j^t)}^2+\dfrac{1}{M}\Ee[\norm{\gg_j^t}^2]\\
    &\leq \norm{\nabla_\btheta \rR^{maml}(\btheta^t;\alpha)+r^t}^2+\dfrac{1}{M}(40\norm{\nabla_\btheta \rR^{maml}(\btheta^t;\alpha)}^2+14V^t+\dfrac{3}{N}V^d) \\
    &\leq 2\rho^2L^2+2\rho^2\alpha^2\mu^2\dfrac{V^d}{N}+ \dfrac{1}{M}\left(40\rho^2L^2+14V^t+\dfrac{3}{N}V^d\right) \\
    &\leq \left(2+\frac{40}{M}\right)\rho^2L^2+\frac{14V^t}{M}+\frac{3V^d(1 + \alpha^2\mu^2M)}{MN}
\end{align*}
where we used $2\rho^2 \leq \sqrt{8} < 3$ following the assumption $\alpha \leq \frac{1}{6\mu}$. For $t=T^{tr}$ to $t=T-1$,
\begin{align*}
    \gg^t &= \frac{1}{N}\sum_{i=1}^{N}\gg(\btheta^t,\xi_i;\gamma)\\
    \Ee(\gg^t) &= \nabla_{\btheta}\rR(\btheta^t;\gamma) \\
    \Ee\norm{\gg^t}^2 &=\norm{\Ee(\gg^t)}^2+\trace(\var(\gg^t)) \leq L^2+V^d/N
\end{align*}


Using the Lipschitz property, $|\rR(\btheta - \alpha \nabla\rR(\btheta;\gamma);\gamma) - \rR(\btheta)| \leq \alpha L^2$, and we can obtain the bound $|\Ee_{\gamma}[\rR(\btheta^{T^{tr}};\gamma)] - \rR^{maml}(\btheta^{T^{tr}})| \leq \alpha L^2$. Therefore, taking the expectation of both sides of ~\eqref{eq:mamltraintest} over $\gg^t$ and $\gamma$ and using $\Ee_\gamma[\rR(\mamlsol-\alpha\nabla_\btheta\rR(\mamlsol;\gamma);\gamma)]=\Lambda^{maml}(\alpha)$,

\begin{equation}
\begin{aligned}
    &\sum_{t=0}^{T^{tr}-1} \norm{\nabla_\btheta \rR^{maml}(\btheta^t;\alpha)}^2 + \sum_{t=0}^{T^{te}-1} \|\nabla_{\btheta}\rR(\btheta^{t+T^{tr}};\gamma)\|_2^2 \\
    &\leq \frac{\Delta + \Lambda^{maml}(\alpha) + \alpha L^2}{\min\{\beta^{tr},\beta^{te}\}}+\sum_{t=0}^{T^{tr}-1}\norm{\nabla_\btheta \rR^{maml}(\btheta^t;\alpha)} \norm{r^t}+\beta^{te}\dfrac{\mu T^{te}(L^2+V^d/N)}{2} \\
    &\quad+\beta^{tr}(2\mu+\mu^h\alpha L)T^{tr} \left(\left(2+\frac{40}{M}\right)\rho^2L^2+\frac{14V^t}{M}+\frac{3V^d(1 + \alpha^2\mu^2M)}{MN}\right)\\
    &\leq \frac{\Delta+\Lambda^{maml}(\alpha)+\alpha L^2}{\min\{\beta^{tr},\beta^{te}\}}+T^{tr}\alpha\mu \rho^2L\sqrt{\frac{V^d}{N}}+\beta^{te}\dfrac{\mu T^{te}(L^2+V^d/N)}{2} \\
    &\quad+\beta^{tr}(2\mu+\mu^H\alpha L)T^{tr}\left(\left(2+\frac{40}{M}\right)\rho^2L^2+\frac{14V^t}{M}+\frac{3V^d(1 + \alpha^2\mu^2M)}{MN}\right)
\end{aligned}
\end{equation}

Assuming $\beta^{tr}=\beta^{te}$ and optimizing the bound over the learning rate, we obtain
\begin{equation}
\begin{aligned}
    &\sum_{t=0}^{T^{tr}-1} \norm{\nabla_\btheta \rR^{maml}(\btheta^t;\alpha)}^2 + \sum_{t=0}^{T^{te}-1} \|\nabla_{\btheta}\rR(\btheta^{t+T^{tr}};\gamma)\|_2^2 \\ &\leq  T^{tr}\alpha\mu \rho^2L\sqrt{V^d/N} +\sqrt{0.5\big(\Delta + \Lambda^{maml}(\alpha)+\alpha L^2\big) \big(C^{maml}_{tr}T^{tr} + C^{maml}_{te}T^{te}\big)}
\end{aligned}
\end{equation}
where
\begin{equation}
    C^{maml}_{tr}= \mu^\prime \left(\left(2+\frac{40}{M}\right)\rho^2L^2+\frac{14V^t}{M}+\frac{3V^d(1 + \alpha^2\mu^2M)}{MN}\right) \text{ and }
C^{maml}_{te}= \mu \left(L^2+\frac{V^d}{N}\right) 
\end{equation}
\end{proof}

==> Neurips2020 (3)/tex/discussion.tex <==
This paper introduces an important trade-off in meta-learning, that of accurately modeling the meta-learning problem and complexity of the optimization problem.
Classic meta-learning algorithms account for the structure of the problem space but define complex optimization objectives.
Domain randomized search (DRS) does not account for the structure of the meta-learning problem and solves a single level optimization objective.

Taking MAML to be the representative meta-learning algorithm, we study this trade-off empirically and theoretically.
On meta-reinforcement learning benchmarks, the optimization complexity appears to be more important; DRS is competitive with and often outperforms MAML, especially for fewer environment steps.
Through an analysis of the sample complexity for smooth nonconvex risk functions, we show that DRS and MAML both solve the meta-learning problem and delineate the roles of optimization complexity and modeling accuracy.
For meta-linear regression, we prove theoretically and verify in simulations that while MAML can utilize the geometry of the distribution of task losses to improve performance through meta-testing optimization, this modeling gain can be counterbalanced by its greater optimization error for small sample sizes.
All three studies show that the balance of the trade-off is not only determined by the sample sizes but characteristics of the meta-learning problem, such as the smoothness of the task risk functions.
%Lastly, we prove that DRS and MAML both solve the meta-learning problem and illustrate the trade-off through a novel analysis of the optimization behavior of both algorithms during meta-training and meta-testing.

There are several interesting directions for future work.
What is the trade-off exhibited by other algorithms, such as Reptile~\citep{reptile} or ANIL~\citep{anil}, that were designed to be more computationally efficient than MAML?
Our theory may also be extended to more complex scenarios such as supervised learning with deep networks, the Linear Quadratic Regulator, more than one inner optimization step in MAML, or the use of part of the data to select hyperparameters.

==> Neurips2020 (3)/tex/linear_reg.tex <==
In this section, we study the linear regression case where we can explicitly characterize the trade-off of optimization error and modeling error.
Since the empirical risk minimization problems corresponding to MAML and DRS in linear regression are analytically solvable, the optimization errors only consist of the statistical errors arising from using empirical risk minimization. 
We first analyze the optimization errors and then discuss the modeling errors of the two approaches. All proofs can be found in Appendix~\ref{sec:linreg_proofs}.

\subsection{Formal Setup and Preliminaries}

For each task $\gamma$, we assume the following data model:
\begin{align}\label{model:lr}
    y_\gamma &= \Thetag\trans \xx_\gamma+\epsilon_\gamma, \quad\quad \epsilon_\gamma \sim (0, \sigmag), \quad\quad \Qg = \Ee[\xx_\gamma \xx_\gamma\trans \mid \gamma].
\end{align}
where $\epsilon_\gamma$ and $\xx_\gamma$ are independent and $\xx_\gamma\in\Re^p$.
We assume the squared error loss;
\begin{equation}\label{eq:lossfunc}
    \lossgt =\dfrac12\Ee[(y_\gamma-\btheta\trans \xx_{\gamma})^2\mid\gamma] = \dfrac12\btheta\trans\Qg\btheta-\Thetag\trans\Qg\btheta+\dfrac12\Thetag\trans\Qg\Thetag+\dfrac12\sigmag.
\end{equation}

The globally optimal (minimum risk) solutions for the DRS and MAML objectives \eqref{eq:objectives} are (\emph{see \ref{app:optimal_sol} for derivations});
\begin{equation}\label{eq:drmamlsols}
    \begin{aligned}
    \drsol &=  \Ee_\gamma[\Qg]^{-1}\Ee_\gamma[\Qg\Thetag] \\
    \mamlsol &=  \Ee_\gamma[(\II-\alpha\Qg)\Qg(\II-\alpha\Qg)]^{-1}\Ee_\gamma[(\II-\alpha\Qg)\Qg(\II-\alpha\Qg)\Thetag].
\end{aligned}
\end{equation}


Both solutions can be viewed as weightings of the task parameters $\Thetag$.
Since the Hessian of $\lossgt$ is $\Qg$, the DRS solution gives greater weight to the tasks whose risk functions have higher curvature, \ie are more sensitive to perturbations in $\btheta$.
Compared to the DRS solution, the MAML solution puts more weight on the tasks with lower curvature.
As the gradient of $\lossgt$ is $\Qg(\btheta-\Thetag)$, for tasks with lower curvature one gradient step on the task risk function takes us a smaller fraction of the distance from the current point $\btheta$ to the stationary point $\Thetag$; thus, starting from the MAML solution enables faster task adaptation overall if the risks are known exactly.

\subsection{Bounds on Optimization Error}

We consider a finite-sample setting where $M$ tasks, independently sampled from $p(\gamma)$ and $2N$ observations per task, sampled according to the model in \eqref{model:lr} are given. We denote the resulting dataset as $\dD \equiv (\xgi,\ygi)$, $j=1,\dots,M, i=1,\dots,2N$.

During meta-training, from~\eqref{eq:empirical_drs_problem}, DRS minimizes the average squared error over all data:
\begin{align}\label{eq:drest}
    \drest &\triangleq \argmin_\btheta \sum_{j=1}^M\sum_{i=1}^{2N}(\ygi-\btheta\trans\xgi)^2.
\end{align}
From~\eqref{eq:maml_empirical}, MAML optimizes for parameters such that, when optimized for each task using SGD on the average squared error over $N$ observations with learning rate $\alpha$, minimizes the average squared error over the remaining $N$ observations of all tasks: 
\begin{align}\label{eq:mamlest}
    \mamlest &\triangleq \argmin_\btheta\sum_{j=1}^M\sum_{i=N+1}^{2N}(\ygi-\tilde{\btheta}_j(\alpha)\trans\xgi)^2, \tilde{\btheta}_j(\alpha)=\btheta-\dfrac{\alpha}{N}\sum_{i=1}^N(\xgi\xgi\trans\btheta-\xgi\ygi)
\end{align}
As a sub-optimality metric, we characterize the distances between the empirical solution and globally optimal solution, $\norm{\drest - \drsol}$ and $\norm{\mamlest - \mamlsol}$, in terms of the finite sample sizes $M$ and $N$ in Theorem~\ref{thm:drbound}\&\ref{thm:mamlbound}. This is the error arising from using empirical samples instead of the population statistics, that is, the statistical error. 

Before we state the theorems, we summarize the assumptions. \textbf{A1:} Bounded Hessian of the task loss, $\norm{\Qg}\leq\beta$. \textbf{A2:} Bounded parameter, feature, and error space, $\norm{\Thetag-\drsol}\leq\tau$, $\norm{\Thetag-\mamlsol}\leq\tau'$ and $\norm{\Thetag}$, $\norm{\xx_{\gamma,i}}$, and $\abs{\epsilon_{\gamma,i}}$ are finite.  \textbf{A3:} The distribution of $\xx_{\gamma,i}$ conditional on $\gamma$ is \textbf{sub-Gaussian} with parameter $K$.
In this setting, the following theorems characterize the statistical error for meta linear-regression.

\begin{theorem}\label{thm:drbound}
Suppose that with probability $1$, \textbf{A1-3} holds. Let $\omega$ be logarithmic in $\delta^{-1}$, $M$, and $p$, and define the functions
\begin{align*}
    & c_1(\Delta,r,s,\theta)=\norm{\theta}\sqrt{2r\Delta}+\sqrt{2s\Delta}, \quad c_2(\Delta)=\beta CK^2\sqrt{p+\Delta}, \quad c_3(\Delta)=\sqrt{\trace(\Ee_\gamma[\sigmag\Qg])\Delta},
\end{align*}
where $C$ is a constant.
If $\lambda_{min}(\Ee_\gamma[\Qg])-\tilde{o}(1)>0$, with probability at least $1-\delta$, ignoring higher order terms, $\norm{\drest-\drsol}$ is bounded above by
\footnote{Here we abuse notation somewhat by defining the variance of a matrix $\BB$ to be $\var(\BB)=\Ee(\BB-\Ee(\BB)^2)$.}
\begin{equation*}
\begin{aligned}
    (\lambda_{min}(\Ee_\gamma[\Qg])-\tilde{o}(1))^{-1}\left(\dfrac{c_1(\omega,\norm{\var_\gamma[\Qg]},\trace(\var_\gamma[\Qg\Thetag]),\drsol)}{\sqrt{M}}+\dfrac{\tau c_2(\omega)/\sqrt{2}+c_3(\omega)}{\sqrt{N}}\right)
\end{aligned}
\end{equation*}
\end{theorem}

\begin{theorem}\label{thm:mamlbound}
With the same assumptions as Theorem~\ref{thm:drbound}, let $\SSS_\gamma(\alpha)=(\II-\alpha\Qg)\Qg(\II-\alpha\Qg)$.
If $\lambda_{min}(\Ee_\gamma[\SSS_\gamma(\alpha)])-\tilde{o}(1)>0$, with probability at least $1-\delta$, ignoring higher order terms, $\norm{\mamlest-\mamlsol}$ is bounded above by
\begin{align*}
    &(\lambda_{min}(\Ee_\gamma[\SSS_\gamma(\alpha)])-\tilde{o}(1))^{-1}\bigg(\dfrac{c_1(\omega,\norm{\var_\gamma[\SSS_\gamma(\alpha)]},\trace(\var_\gamma[\SSS_\gamma(\alpha)\Thetag]),\mamlsol)}{\sqrt{M}} \\
    &\hspace{4.5cm}+\dfrac{(1+3\alpha\beta)^2\tau'c_2(\omega)+\sqrt{2}(1+\alpha\beta)^2 c_3(\omega)}{\sqrt{N}}\bigg).
\end{align*}
\end{theorem}

Theorems \ref{thm:drbound}\&\ref{thm:mamlbound} show the statistical errors for MAML and DRS scale similarly in terms of rates with respect to $N$ and $M$. However, the constants are significantly different. Compare the coefficients of $\nicefrac{1}{\sqrt{N}}$.
The coefficient of $c_2(\omega)$ for DRS is $\tau\sqrt{2}^{-1}\lambda_{min}(\Ee_\gamma[\Qg])^{-1}$ and for MAML it is $\tau'(1+3\alpha\beta)^2\lambda_{min}(\Ee_\gamma[\SSS_\gamma(\alpha)])^{-1}$.
When $\alpha\beta\lessapprox 1$, the latter is larger than the former, since we expect that $\tau \approx \tau'$ and the eigenvalues of $\Ee_\gamma[\SSS_\gamma(\alpha)]$ to be shrunken compared to those of $\Ee_\gamma[\Qg]$.
A similar observation holds for the coefficient of $c_3(\omega)$. In other words, the convergence behavior of the MAML estimate has a worse dependence on $N$, indicating that the statistical error for DRS has more favorable behavior.

\subsection{Modeling Error}

Modeling error affects the meta-testing performance of the globally optimal solutions. We expect MAML to perform better as it directly models the meta-learning problem whereas DRS does not. Modeling error by definition depends on the correct model of the world and thus is difficult to characterize without domain knowledge. We study this error in the following theorem assuming that the distribution of tasks is the same for meta-training and meta-testing and discuss its implications for practitioners.

\begin{theorem}\label{thm:loss}
For meta-test task $\gamma$ and arbitrary $\btheta$, let $\tilde{\btheta}_{\gamma}(\alpha)$ be the parameters optimized by one step of SGD using $N$ data points $\oO_\gamma$ and learning rate $\alpha$, as in~\eqref{eq:mamlest}.
Let $\Ag=\SSS_\gamma(\alpha)+\alpha^2(\Ee[\xx_{\gamma,i}\xx_{\gamma,i}\trans\Qg \xx_{\gamma,i}\xx_{\gamma,i}\trans]-\Qg^3)/N$, where $\SSS_\gamma(\alpha)$ is defined in Theorem~\ref{thm:mamlbound}.
The expected losses before and after optimization, as functions of $\btheta$, are
\begin{align*}
    \rR^{drs}(\btheta) &\equiv \Ee_\gamma\left[\norm{\btheta-\Thetag}_{\Qg}^2\right] \quad \text{and} \quad \Ee_\gamma[\Ee_{\oO_\gamma}[\rR(\tilde{\btheta}_{\gamma}(\alpha);\gamma)]] \equiv \Ee_\gamma\left[\norm{\btheta-\Thetag}_{\Ag}^2\right],
\end{align*}
where we have ignored constants and terms that do not include $\btheta$.
The former is minimized by $\drsol$.
As $N\to\infty$, the latter approaches $\rR^{maml}(\btheta;\alpha)$, is minimized by $\mamlsol$ and, for $0<\alpha\leq 1/\beta$, is at most $\rR^{drs}(\drsol)$, the minimum expected loss possible before meta-testing optimization.
\end{theorem}

Theorem~\ref{thm:loss} shows that the smaller modeling error of meta-learning indeed translates to improved performance. 
Meta-learning can utilize the geometry implied by the distribution of the tasks to reduce the expected loss given the ability to optimize at meta-testing.

%In the asymptotic regime where $M\to\infty$ and $N\to\infty$, by Theorems~\ref{thm:drbound}\&\ref{thm:mamlbound}, $\drest\p\drsol$ and $\mamlest\p\mamlsol$, i.e. the statistical errors of the DRS and MAML estimates are zero. 
%By Theorem~\ref{thm:loss}, the DRS estimate would be superior to the MAML estimate before test time adaptation and the MAML estimate superior to the DRS estimate after test time adaptation, with the MAML estimate after test time adaptation being the best overall. However, when $\beta$ is large, the worse dependence of the statistical error for MAML on $N^{-1/2}$ suggests that for small $N$, the DRS estimate may have smaller expected loss than the MAML estimate before \emph{and} after adaptation.


Combining the results of all theorems, the optimization error is worse for MAML when $\alpha\beta\lessapprox 1$ from Theorem \ref{thm:drbound}\&\ref{thm:mamlbound}. DRS does not model the meta structure, hence it has worse modeling error/greater expected loss by Theorem~\ref{thm:loss}. As expected, there is no clear winner in practice as the choice depends on the trade-off between optimization error and modeling error. Next, we show this empirically.


\subsection{Empirical Results}
We carried out simulations to empirically study the trade-off in the linear regression case. We chose the following specific distribution of tasks and data model:
\begin{align}\label{model:lrsimulation}
    \begin{split}
    y_\gamma &= \Thetag\trans \xx_\gamma+\epsilon_\gamma \quad\quad \epsilon_\gamma \sim \nN(0, \sigmag) \quad\quad \xx_\gamma\sim \nN(0,\Qg) \\
    \Thetag &\sim U([0,2]^p) \quad\quad \sigmag\sim U([0,2]) \quad\quad \Qg=\VV\diag(\Thetag)\VV^T \quad\quad \VV\sim U(\mathds{SO}(p))
    \end{split}
\end{align}

We present the case for $p=1$; larger $p$ lead to similar qualitative results. We compute approximations of $\rR^{drs}(\btheta)$ (expected loss before meta-testing optimization) as a function of $\btheta$ and $\Ee_\gamma[\Ee_{\oO_\gamma}[\rR(\gamma;\tilde{\btheta}_{\gamma}(\alpha))]$ (expected loss after meta-testing optimization) as a function of $\btheta$ and $\alpha$.
For various $M$ and $N$, we generate a collection of datasets $\dD$; for each $\dD$, over a grid of values for $\alpha\in [0,1]$, we compute the corresponding DRS and MAML estimates and, using the aforementioned functions, calculate whether the MAML estimate has lower expected loss than the DRS estimate before and after meta-testing optimization. Figure~\ref{fig:p1} shows contour plots of the fraction of the datasets for which the MAML estimate has lower expected loss before meta-testing optimization (left three figures) and after (right three figures), for several values of $\alpha$.
The axes are the number of tasks ($M$) and the data set size for meta-testing optimization ($N$).

\begin{figure}[tbh]
    \includegraphics[width=\textwidth]{figures/meta_lr_a4.pdf}
    \caption{$p=1$: Contour plots of the probability that the MAML estimate has lower expected loss than the DR estimate before meta-testing optimization (pre) and after (post). The axes are the number of tasks ($M$) and the number of data points used for meta-testing optimization ($N$), and $\alpha$ is fixed.}
    \label{fig:p1}
\end{figure}


From Figure~\ref{fig:p1}, for very high $M$ and $N$, the DRS estimate has lower expected loss before meta-testing optimization and the MAML estimate has lower expected loss after meta-testing optimization with very high certainty. This is expected as asymptotically meta-learning is expected to work well by Theorem~\ref{thm:loss}; the practical question of interest is the finite sample case.

From Figure~\ref{fig:p1}-post, we observe that for small $M$ and $N$, the probability that the MAML estimate has lower expected loss after meta-testing optimization can be substantially lower than $0.5$, \ie the DRS estimate is superior.
%In addition, the thresholds of $M$ and $N$ beyond which the MAML estimate has lower expected loss after test time adaptation with high probability are higher for more extreme values of $\alpha$.
We conclude that in this case the increased optimization error from MAML dominates the decreased modeling error. Hence, unless the geometry is strongly skewed, DRS is desirable for smaller datasets in meta-linear regression.



\iffalse
\begin{lemma}\label{lem:lossfunc}
For task $\gamma$, the loss as a function of $\theta$ is
\begin{align*}
    \lossgt &=\dfrac12\Ee[(y_\gamma-\theta\trans x_{\gamma})^2\mid\gamma] = \dfrac12\theta\trans\Qg\theta-\Thetag\trans\Qg\theta+\dfrac12\Thetag\trans\Qg\Thetag+\dfrac12\sigmag.
\end{align*}
\end{lemma}
\begin{proposition}\label{prop:drmamlsols}
Define $\drsol=\argmin_\theta \Ee_\gamma[\lossgt]$ and for $\alpha>0$, $\mamlsol=\argmin_\theta \Ee_\gamma[\mamllossgt]$.
Then,
\begin{align*}
    \drsol &= \Ee_\gamma[\Qg]^{-1}\Ee_\gamma[\Qg\Thetag] \\
    \mamlsol &= \Ee_\gamma[(I-\alpha\Qg)\Qg(I-\alpha\Qg)]^{-1}\Ee_\gamma[(I-\alpha\Qg)\Qg(I-\alpha\Qg)\Thetag].
\end{align*}
\end{proposition}
\fi 





\iffalse
We study a ERM scenario that mimics practical algorithms for DR and MAML.

Suppose that there are a set of $M$ tasks, independently sampled from the distribution $p(\gamma)$. 
For each task, there are $2N$ observations independently sampled according to Model~\ref{model:lr}: 

\begin{theorem}\label{thm:drbound}
Suppose that with probability $1$, $\norm{\Qg}\leq\beta$, $\norm{\Thetag-\drsol}\leq\tau$ and $\norm{\Thetag}$, $\norm{x_{\gamma,i}}$, and
$\abs{\epsilon_{\gamma,i}}$ are bounded, and that the distribution of $x_{\gamma,i}$ conditional on $\gamma$ is sub-Gaussian with parameter $K$.
Then, as $M, N \to \infty$, $\drest \p \drsol$.

More explicitly, let $\omega$ be logarithmic in $\delta^{-1}$, $M$, and $p$, and define the functions
\katelyn{These definitions can be moved to the supplement if necessary for space. I've kept them for now since they do have informative value.}
\begin{align*}
    & c_1(\Delta,r,s,\theta)=\norm{\theta}\sqrt{2r\Delta}+\sqrt{2s\Delta} \\
    & c_2(\Delta)=\beta CK^2\sqrt{p+\Delta} \quad \text{where $C$ is a constant} \\
    & c_3(\Delta)=\sqrt{\trace(\Ee_\gamma[\sigmag\Qg])\Delta}.
\end{align*}
If $\lambda_{min}(\Ee_\gamma[\Qg])-\tilde{o}(1)>0$, with probability at least $1-\delta$, ignoring higher order terms, $\norm{\drest-\drsol}$ is bounded above by
\begin{align*}
    &(\lambda_{min}(\Ee_\gamma[\Qg])-\tilde{o}(1))^{-1}\left(\dfrac{c_1(\omega,\norm{\var_\gamma[\Qg]},\trace(\var_\gamma[\Qg\Thetag]),\drsol)}{\sqrt{M}}+\dfrac{\tau c_2(\omega)/\sqrt{2}+c_3(\omega)}{\sqrt{N}}\right).
\end{align*}
\end{theorem}


\mypara{Remark.}

At test time, given a new task $\gamma$ and $N$ observations $\oO_{\gamma}\equiv \{(x_{\gamma,i},y_{\gamma,i})\}_{i=1}^N$, $\drest$ and $\mamlest$ are adapted using SGD on the average squared error over the observations with learning rate $\alpha$ to $\tilde{\theta}_{DR,\gamma}$ and $\tilde{\theta}_{MAML,\gamma}(\alpha)$. More explicitly, the following formula is used for arbitrary $\theta$:
\begin{align*}
    &\tilde{\theta}_{\gamma}(\alpha)=\theta-\dfrac{\alpha}{N}\sum_{i=1}^N(x_{\gamma,i}x_{\gamma,i}\trans\theta-x_{\gamma,i}y_{\gamma,i}).
\end{align*}

As in Section~\ref{sec:metarlexp}, we consider the case where test tasks are assumed to be sampled from $p(\gamma)$ as well.

\subsection{Simulations of ERM scenario}

% We purposefully chose the distributions of $\Thetag$ and $\Qg$ to be dependent; if they are independent, from Proposition~\ref{prop:drmamlsols} $\drsol=\mamlsol=\Ee_\gamma[\Thetag]$, so we should expect the DR and MAML estimates to behave similarly for large $M$ and $D$.

\begin{figure}
    \centering
    \begin{subfigure}[b]{0.32\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/p1pre_alpha25.png}
        \caption{$\alpha=0.25$, before}
        \label{fig:prealpha25}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.32\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/p1pre_alpha50.png}
        \caption{$\alpha=0.50$, before}
        \label{fig:prealpha50}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.32\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/p1pre_alpha75.png}
        \caption{$\alpha=0.75$, before}
        \label{fig:prealpha75}
    \end{subfigure}
    \\
    \begin{subfigure}[b]{0.32\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/p1post_alpha25.png}
        \caption{$\alpha=0.25$, after}
        \label{fig:postalpha25}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.32\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/p1post_alpha50.png}
        \caption{$\alpha=0.50$, after}
        \label{fig:postalpha50}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.32\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/p1post_alpha75.png}
        \caption{$\alpha=0.75$, after}
        \label{fig:postalpha75}
    \end{subfigure}
    \caption{$p=1$: Contour plots of the probability that the MAML estimate has lower expected loss than the DR estimate before test time adaptation (left column) and after (right column). The axes are the number of tasks ($M$) and the size of the support and query sets ($N$), and $\alpha$ is fixed.}
    \label{fig:p1}
\end{figure}
\fi




\iffalse
\begin{figure}[tbh]
\begin{tabular}{@{}c@{\hspace{1mm}}c@{\hspace{1mm}}c@{\hspace{1mm}}c@{\hspace{1mm}}c@{\hspace{1mm}}c@{}}
\multicolumn{6}{@{}c@{}}{\includegraphics[width=\textwidth]{figures/colorbar.pdf}} \\
        \includegraphics[width=0.16\textwidth]{figures/preupdate_alpha_25.pdf} & 
        \includegraphics[width=0.16\textwidth]{figures/preupdate_alpha_50.pdf} &
        \includegraphics[width=0.16\textwidth]{figures/preupdate_alpha_75.pdf} &
        \includegraphics[width=0.16\textwidth]{figures/postupdate_alpha_10.pdf} &
        \includegraphics[width=0.16\textwidth]{figures/postupdate_alpha_25.pdf} &
        \includegraphics[width=0.16\textwidth]{figures/postupdate_alpha_75.pdf} \\
        $\alpha=0.25$, pre & $\alpha=0.5$,  pre & $\alpha=0.75$, pre & $\alpha=0.1$, post & $\alpha=0.25$,  post & $\alpha=0.75$, post \\
    \end{tabular}
    \caption{$p=1$: Contour plots of the probability that the MAML estimate has lower expected loss than the DR estimate before test time optimization (pre) and after (post). The axes are the number of tasks ($M$) and the number of data points used for test time optimization ($N$), and $\alpha$ is fixed.}
    \label{fig:p1}
\end{figure}
\fi 

==> Neurips2020 (3)/tex/linreg_proofs.tex <==
\subsection{Derivation for risk function in Equation~\ref{eq:lossfunc}}
\label{app:risk_func}

\begin{align*}
    \lossgt &=\dfrac12\Ee[(y_\gamma-\btheta\trans \xx_\gamma)^2 \mid \gamma] \\
    &= \dfrac12\Ee[(\epsilon_\gamma+(\Thetag-\btheta)\trans \xx_\gamma)^2 \mid \gamma] \\
    &= \dfrac12\Ee[\epsilon_\gamma^2+2(\Thetag-\btheta)\trans \xx_\gamma\epsilon_\gamma+(\Thetag-\btheta)\trans \xx_\gamma \xx_\gamma\trans(\Thetag-\btheta) \mid \gamma] \\
    &=\dfrac12[\sigmag+(\Thetag-\btheta)\trans\Qg(\Thetag-\btheta)] \\
    &=\dfrac12\btheta\trans\Qg\btheta-\Thetag\trans\Qg\btheta+\dfrac12\Thetag\trans\Qg\Thetag+\dfrac12\sigmag
\end{align*}
where the third equality uses the model~\eqref{model:lr}.


\subsection{Derivation for optimal solutions in Equation~\ref{eq:drmamlsols}}
\label{app:optimal_sol}

Recall that $\drsol\triangleq\argmin_\theta \Ee_\gamma[\lossgt]$ and $\mamlsol\triangleq\argmin_\theta \Ee_\gamma[\mamllossgt]$.
Using Equation~\ref{eq:lossfunc},
\begin{align*}
    \Ee_\gamma[\lossgt] &= \Ee_\gamma[\dfrac12\btheta\trans\Qg\btheta-\Thetag\trans\Qg\btheta+\dfrac12\Thetag\trans\Qg\Thetag+\dfrac12\sigmag] \\
    &= \dfrac12\btheta\trans\Ee_\gamma[\Qg]\btheta-\Ee_\gamma[\Qg\Thetag]\trans\btheta+\dfrac12\Ee_\gamma[\Thetag\trans\Qg\Thetag]+\dfrac12\Ee_\gamma[\sigmag] \\
    \nabla_\theta\Ee_\gamma[\lossgt] &= \Ee_\gamma[\Qg]\btheta-\Ee_\gamma[\Qg\Thetag]
\end{align*}
Since $\Ee_\gamma[\lossgt]$ is quadratic in $\btheta$, it is minimized at a first-order stationary point.
Thus, setting $\nabla_\theta\Ee_\gamma[\lossgt]$ equal to zero, we obtain $\drsol=\Ee_\gamma[\Qg]^{-1}\Ee_\gamma[\Qg\Thetag]$. 

Similarly,
\begin{align*}
    &\Ee_\gamma[\mamllossgt] \\
    &=\Ee_\gamma[\rR(\btheta-\alpha(\Qg\btheta-\Qg\Thetag);\gamma)] \\
    &=\Ee_\gamma[\rR((\II-\alpha\Qg)\btheta+\alpha\Qg\Thetag;\gamma)] \\
    &=\dfrac12\Ee_\gamma[((\II-\alpha\Qg)\btheta+\alpha\Qg\Thetag)\trans\Qg((\II-\alpha\Qg)\btheta+\alpha\Qg\Thetag)] \\
    &\quad-\Ee_\gamma[\Thetag\trans\Qg((\II-\alpha\Qg)\btheta+\alpha\Qg\Thetag)]+\dfrac12\Ee_\gamma[\Thetag\trans\Qg\Thetag]+\dfrac12\Ee_\gamma[\sigmag] \\
    &=\dfrac12\btheta\trans\Ee_\gamma[(\II-\alpha\Qg)\Qg(\II-\alpha\Qg)]\btheta-\Ee_\gamma[\Thetag\trans(\II-\alpha\Qg)\Qg(\II-\alpha\Qg)]\btheta\\
    &\quad+\dfrac12\Ee_\gamma[\Thetag\trans(\II-\alpha\Qg)\Qg(\II-\alpha\Qg)\Thetag]+\dfrac12\Ee_\gamma[\sigmag] \\
    &\nabla_\theta\Ee_\gamma[\mamllossgt] \\
    &= \Ee_\gamma[(\II-\alpha\Qg)\Qg(\II-\alpha\Qg)]\btheta-\Ee_\gamma[(\II-\alpha\Qg)\Qg(\II-\alpha\Qg)\Thetag]
\end{align*}
$\Ee_\gamma[\mamllossgt]$ is also quadratic in $\btheta$, so we obtain its minimizer by setting its gradient equal to zero.
Thus, $\mamlsol=\Ee_\gamma[(\II-\alpha\Qg)\Qg(\II-\alpha\Qg)]^{-1}\Ee_\gamma[(\II-\alpha\Qg)\Qg(\II-\alpha\Qg)\Thetag]$.


\subsection{Proof of Theorem~\ref{thm:drbound} and \ref{thm:mamlbound}}
\subsubsection{Useful Lemmas and Preliminary Results}
We start with stating a few useful lemmas to be used in the proof of the main statements. Following them, we analyze $\drest$ and $\mamlest$.

\begin{lemma}\label{prop:drestmamlest}
Let $\XX_{j1}$ be the $p\times N$ matrix with columns $\xgi, i=1,\dots,N$ and $\XX_{j2}$ be the $p\times N$ matrix with columns $\xgi, i=N+1,\dots,2N$. 
Let $\YY_{j1}$ be the $N$-dimensional vector with entries $\ygi, i=1,\dots,N$, and $\YY_{j2}$ be the $N$-dimensional vector with entries $\ygi, i=N+1,\dots,2N$.
Let $\XX=\begin{bmatrix}\dots & \XX_{j1} & \XX_{j2} & \dots\end{bmatrix}$ and $\YY=\begin{bmatrix}\dots & \YY_{j1}\trans & \YY_{j2}\trans &\dots\end{bmatrix}\trans$.
Let $\WW(\alpha)=\begin{bmatrix}\dots & (\II-\dfrac{\alpha}{N}\XX_{j1}\XX_{j2}\trans)\XX_{j2} & \dots\end{bmatrix}$ and $\ZZ(\alpha)=\begin{bmatrix} \dots & (\YY_{j2}-\dfrac{\alpha}{N}\XX_{j2}\trans\XX_{j1}\YY_{j1})\trans & \dots\end{bmatrix}\trans$.
Then,
\begin{align*}
    \drest &= (\XX\trans)^+\YY \quad\text{and}\quad \mamlest = (\WW(\alpha)\trans)^+\ZZ(\alpha)
\end{align*}
where $()^+$ denotes the Moore-Penrose pseudoinverse of a matrix.
\end{lemma}
\begin{proof}
Using~\eqref{eq:drest}, we can write the DR estimate as minimizing the objective
\begin{align*}
    \dfrac{1}{4MN}\sum_{j=1}^M\sum_{i=1}^{2N}(\ygi-\btheta\trans \xgi)^2 &=\dfrac{1}{4MN}\sum_{j=1}^M\left(\|\YY_{j1}-\XX_{j1}^T\btheta\|_2^2+\|\YY_{j2}-\XX_{j2}\trans\btheta\|_2^2\right) \\
    &=\dfrac{1}{4MN}\|\YY-\XX\trans\btheta\|_2^2
\end{align*}
From \citet{penrose}, the value of $\btheta$ that minimizes the above is $(\XX\trans)^+\YY$.

Using~\eqref{eq:mamlest}, we can write the MAML estimate as minimizing the objective
\begin{align*}
    &\dfrac{1}{2MN}\sum_{j=1}^M\sum_{i=N+1}^{2N}(\ygi-\tilde{\btheta}_j(\alpha)\trans \xgi)^2 \\
    &= \dfrac{1}{2MN}\sum_{j=1}^M \|\YY_{j2}-\XX_{j2}\trans\tilde{\btheta}_j(\alpha)\|_2^2 \\
    &= \dfrac{1}{2MN}\sum_{j=1}^M \|\YY_{j2}-\XX_{j2}\trans(\btheta-\dfrac{\alpha}{N}(\XX_{j1}\XX_{j1}\trans\btheta-\XX_{j1}\YY_{j1}))\|_2^2 \\
    &= \dfrac{1}{2MN}\sum_{j=1}^M\|\YY_{j2}-\dfrac{\alpha}{N}\XX_{j2}\trans\XX_{j1}\YY_{j1}-((\II-\dfrac{\alpha}{N}\XX_{j1}\XX_{j1}^T)\XX_{j2})\trans\btheta\|_2^2 \\
    &= \dfrac{1}{2MN}\|\ZZ(\alpha)-\WW(\alpha)\trans\btheta\|_2^2
\end{align*}
With the same reasoning as for the DR estimate, this is minimized when $\btheta$ equals $(\WW(\alpha)\trans)^+\ZZ(\alpha)$.
\end{proof}


Next, we obtain some useful high probability concentration inequalities as a direct consequence of matrix Bernstein's inequality~\citep{hdpbook}.
\begin{lemma}\label{lem:qghpbound}
Assume $\norm{\Qg}\leq\beta$ with probability $1$. With probability at least $1-\varrho$,
\begin{align*}
\norm{\sum_{j=1}^M(\QQ_j-\Ee_\gamma[\Qg])}\leq \dfrac{2\beta}{3}\log{\frac{2p}{\varrho}}+\sqrt{2M\norm{\var_\gamma[\Qg]}\log{\frac{2p}{\varrho}}}
\end{align*}
\end{lemma}
\begin{proof}
Notice that $\QQ_j-\Ee_\gamma[\Qg]$ are $M$ independent, mean zero, symmetric random matrices.
From the matrix Bernstein's inequality~\citep{hdpbook}, for any $t\geq 0$, 
\begin{align*}
    &\Pe\left\{\left\|\sum_{j=1}^M (\QQ_j-\Ee_\gamma[\Qg])\right\|\geq t\right\}\leq 2p\exp\left\{-\dfrac{t^2/2}{s_1^2+\beta t/3}\right\}
\end{align*}
where
\begin{align*}
    &s_1^2=\norm{\sum_{j=1}^M\Ee[(\QQ_j-\Ee_\gamma[\Qg])^2]}\leq M\norm{\Ee_\gamma[(\Qg-\Ee_\gamma[\Qg])^2]}=M\norm{\var_\gamma[\Qg]}.
\end{align*}
Therefore,
\begin{align*}
    &\Pe\left\{\norm{\sum_{j=1}^M (\QQ_j-\Ee_\gamma[\Qg])}\geq t\right\}\leq 2p\exp\left\{-\dfrac{t^2/2}{M\norm{\var_\gamma[\Qg]}+\beta t/3}\right\}.
\end{align*}
Setting $\omega=\dfrac{t^2/2}{M\norm{\var_\gamma[\Qg]}+\beta t/3}$, we solve for $t$. 
$t$ satisfies the quadratic equation $3t^2-2\beta\omega t-6M\norm{\var_\gamma[\Qg]}\omega=0$, which has the positive root $(\beta\omega+\sqrt{\beta^2\omega^2+18M\norm{\var_\gamma[\Qg]}\omega})/3$.
Therefore, the previous inequality becomes
\begin{align*}
    &\Pe\{\norm{\sum_{j=1}^M (\QQ_j-\Ee_\gamma[\Qg])}\geq \dfrac{\beta\omega+\sqrt{\beta^2\omega^2+18M\norm{\var_\gamma[\Qg]}\omega}}{3}\}\leq 2p\exp\{-\omega\}
    \end{align*}
and since $(\beta\omega+\sqrt{\beta^2\omega^2+18M\norm{\var_\gamma[\Qg]}\omega})/3\leq2\beta\omega/3+\sqrt{2M\norm{\var_\gamma[\Qg]}\omega}$,
\begin{align*}
    &\Pe\{\norm{\sum_{j=1}^M (\QQ_j-\Ee_\gamma[\Qg])}\geq \dfrac{2\beta\omega}{3}+\sqrt{2M\norm{\var_\gamma[\Qg]}\omega}\}\leq 2p\exp\{-\omega\}.
\end{align*}
Set $w=\log{\frac{2p}{\varrho}}$ to obtain the final result.
\end{proof}
\mypara{Remark.} A similar proof will also show that if $\norm{\Qg}\leq\beta$ and $\norm{\II-\alpha\Qg}\leq\mu$ with probability $1$, $\norm{\sum_{j=1}^M((\II-\alpha \QQ_j)\QQ_j(\II-\alpha \QQ_j)-\Ee_\gamma[(\II-\alpha\Qg)\Qg(\II-\alpha\Qg)])}\leq\dfrac{2\beta\mu^2}{3}\log{\frac{2p}{\varrho}}+\sqrt{2M\norm{\var_\gamma[(\II-\alpha\Qg)\Qg(\II-\alpha\Qg)]}\log{\frac{2p}{\varrho}}}$ with probability $1-\varrho$.
\vspace{\baselineskip}

\begin{lemma}\label{lem:qgtghpbound}
Assume $\norm{\Qg}\leq\beta$ and $\norm{\Thetag}\leq\eta$ with probability $1$. With probability at least $1-\varrho$,
\begin{align*}
    \norm{\sum_{j=1}^M(\QQ_j\tasktheta-\Ee_\gamma[\Qg\Thetag])} \leq \dfrac{2\beta\eta}{3}\log{\frac{2(p+1)}{\varrho}}+ \sqrt{2M\trace(\var_\gamma[\Qg\Thetag])\log{\frac{2(p+1)}{\varrho}}}
\end{align*}
\end{lemma}
\begin{proof}
Notice that $\QQ_j\tasktheta-\Ee_\gamma[\Qg\Thetag]$ are $M$ independent, mean zero, random vectors. 
From the matrix Bernstein's inequality for rectangular matrices~\citep{hdpbook}, since $\norm{\Qg\Thetag}\leq\norm{\Qg}\norm{\Thetag}\leq\beta\eta$, for any $t\geq 0$,
\begin{align*}
&\Pe\left\{\norm{\sum_{j=1}^M (\QQ_j\tasktheta-\Ee_\gamma[\Qg\Thetag])}\geq t\right\}\leq 2(p+1)\exp\left\{-\dfrac{t^2/2}{s_2^2+\beta\eta t/3}\right\}
\end{align*}
where
\begin{align*}
    s_2^2&=\max\left(\norm{\sum_{j=1}^M\Ee[(\QQ_j\tasktheta-\Ee_\gamma[\Qg\Thetag])(\QQ_j\tasktheta-\Ee_\gamma[\Qg\Thetag])\trans]},\right. \\
    &\left.\quad\quad\quad\quad\norm{\sum_{j=1}^M\Ee[(\QQ_j\tasktheta-\Ee_\gamma[\Qg\Thetag])\trans(\QQ_j\tasktheta-\Ee_\gamma[\Qg\Thetag])]}\right) \\
    &\leq M\max(\norm{\Ee_\gamma[(\Qg\Thetag-\Ee_\gamma[\Qg\Thetag])(\Qg\Thetag-\Ee_\gamma[\Qg\Thetag])\trans]}, \\
    &\quad\quad\quad\quad\quad\norm{\Ee_\gamma[(\Qg\Thetag-\Ee_\gamma[\Qg\Thetag])\trans(\Qg\Thetag-\Ee_\gamma[\Qg\Thetag])]}) \\
    &=M\max(\norm{\var_\gamma[\Qg\Thetag]},\norm{\trace(\var_\gamma[\Qg\Thetag])}) \\
    &\leq M\trace(\var_\gamma[\Qg\Thetag])
\end{align*}
Therefore,
\begin{align*}
    &\Pe\left\{\norm{\sum_{j=1}^M (\QQ_j\tasktheta-\Ee_\gamma[\Qg\Thetag])}\geq t\right\}\leq 2(p+1)\exp\left\{-\dfrac{t^2/2}{M\trace(\var_\gamma[\Qg\Thetag])+\beta\eta t/3}\right\}.
\end{align*}
Using the same argument as in the proof of Lemma~\ref{lem:qghpbound}, we have that
\begin{align*}
    &\Pe\left\{\norm{\sum_{j=1}^M (\QQ_j\tasktheta-\Ee_\gamma[\Qg\Thetag])}\geq \dfrac{2\beta\eta\omega}{3}+\sqrt{2M\trace(\var_\gamma[\Qg\Thetag])\omega}\right\}\leq 2(p+1)\exp\{-\omega\}.
\end{align*}
Set $w=\log{\frac{2(p+1)}{\varrho}}$ to obtain the final result.

\end{proof}
\mypara{Remark.} A similar argument will also show that if $\norm{\Qg}\leq\beta$, $\norm{\II-\alpha\Qg}\leq\mu$, and $\norm{\Thetag}\leq\eta$,
$\norm{\sum_{j=1}^M((\II-\alpha \QQ_j)\QQ_j(\II-\alpha \QQ_j)\tasktheta-\Ee_\gamma[(\II-\alpha\Qg)\Qg(\II-\alpha\Qg)\Thetag])}\leq\dfrac{2\beta\mu^2\eta}{3}\log{\frac{2(p+1)}{\varrho}}+\sqrt{2M\trace(\var_\gamma[(\II-\alpha\Qg)\Qg(\II-\alpha\Qg)\Thetag])\log{\frac{2(p+1)}{\varrho}}}$ with probability at least $1-\varrho$.
\vspace{\baselineskip}

\begin{lemma}\label{lem:covbound}
Fix the task $j$. Assume $\norm{\Qg}\leq\beta$ with probability $1$ and the distribution of $\xx_{\gamma,i}$ conditional on $\gamma$ is sub-Gaussian with parameter $K$. With probability at least $1-\varrho$,
\begin{align*}
\norm{\dfrac{\XX_{j1}\XX_{j1}\trans}{N}-\QQ_j}\leq \beta CK^2\left(\sqrt{\dfrac{p+\log{\frac{2}{\varrho}}}{N}}+\dfrac{p+\log{\frac{2}{\varrho}}}{N}\right)
\end{align*}
\end{lemma}
\begin{proof}
From results on covariance estimation from~\citet{hdpbook},
\begin{align*}
    &\Pe\{\norm{\dfrac{\XX_{j1}\XX_{j1}\trans}{N}-\QQ_j}\geq CK^2(\sqrt{\dfrac{p+\omega}{N}}+\dfrac{p+\omega}{2N})\norm{\QQ_j}\}\leq 2\exp\{-\omega\}.
\end{align*}
Since $\QQ_j\leq\beta$ with probability $1$,
\begin{align*}
    &\Pe\{\norm{\dfrac{\XX_{j1}\XX_{j1}\trans}{N}-\QQ_j}\geq \beta CK^2(\sqrt{\dfrac{p+\omega}{N}}+\dfrac{p+\omega}{N})\}\leq 2\exp\{-\omega\}.
\end{align*}
Set $w=\log{\frac{2}{\varrho}}$ to obtain the final result.
\end{proof}

\begin{lemma}\label{lem:xgegbound}
Fix the task $j$ and let $\ee_{j1}$ be the $N$-dimensional vector with entries $\epsilon_{j,i},i=1,\dots,N$. If $\norm{\xx_{\gamma,i}}\leq\xi$ and $\abs{\epsilon_{\gamma,i}}\leq\phi$ with probability $1$,
$\norm{\XX_{j1}\ee_{j1}}\geq\dfrac{2\xi\phi\omega}{3}+\sqrt{2N\trace(\Ee_\gamma[\sigmag\Qg])\omega}$ with probability at most $2(p+1)e^{-\omega}$.
\end{lemma}
\begin{proof}
Notice that $\XX_{j1}\ee_{j1}=\sum_{i=1}^{N}\xgi\epsilon_{j,i}$ is the sum of $N$ independent, mean zero, random vectors.
From the matrix Bernstein's inequality for rectangular matrices, for any $t\geq 0$,
\begin{align*}
    &\Pe\{\norm{\XX_{j1}\ee_{j1}} \geq t\} \leq 2(p+1)\exp\{-\dfrac{t^2}{s_3^2+\xi\phi t/3}\}
\end{align*}
for
\begin{align*}
    s_3^2 &= \max(\norm{\sum_{i=1}^{N}\Ee[\xgi\epsilon_{j,i}^2\xgi\trans]},\norm{\sum_{i=1}^{N}\Ee[\epsilon_{j,i}\xgi\trans\xgi\epsilon_{j,i}]}) \\
    &\leq N\max(\norm{\Ee_\gamma[\sigmag\Qg]},\norm{\Ee_\gamma[\sigmag\Ee[\xx_{\gamma,i}\trans \xx_{\gamma,i}\mid\gamma]]}) \\
    &= N\max(\norm{\Ee_\gamma[\sigmag\Qg]},\norm{\Ee_\gamma[\sigmag \trace(\Qg)]}) \\
    &= N\max(\norm{\Ee_\gamma[\sigmag\Qg]},\trace(\Ee_\gamma[\sigmag\Qg])) \\
    &= N \trace(\Ee_\gamma[\sigmag\Qg])
\end{align*}
where the last equality follows from the fact that for a symmetric positive semidefinite matrix such as $\Ee_\gamma[\sigmag\Qg]$, the norm is the largest eigenvalue and the trace is the sum of the eigenvalues.
Therefore,
\begin{align*}
    &\Pe\{\norm{\XX_{j1}\ee_{j1}}\geq t\}\leq 2(p+1)\exp\{-\dfrac{t^2/2}{N\trace(\Ee_\gamma[\sigmag\Qg])+\xi\phi t/3}\}.
\end{align*}
Using the same argument as Lemma~\ref{lem:qghpbound}, we have that
\begin{align*}
    &\Pe\{\norm{\XX_{j1}\ee_{j1}}\geq \dfrac{2\xi\phi\omega}{3}+\sqrt{2N\trace(\Ee_\gamma[\sigmag\Qg])\omega}\}\leq 2(p+1)\exp\{-\omega\}.
\end{align*}
\end{proof}

\subsubsection{Proof of Theorem~\ref{thm:drbound}}

\begin{proof}
Let $\XX_j=\begin{bmatrix}\XX_{j1} & \XX_{j2} \end{bmatrix}$ and
$\YY_j = \begin{bmatrix}\YY_{j1}\trans & \YY_{j2}\trans\end{bmatrix}\trans$.
Let $\ee_{j}$ be the $2N$-dimensional vector with entries $\epsilon_{j,i}, i=1,\dots,2N$.
Let the singular value decomposition of $\XX$ be $UDV\trans$.
Then, from Proposition~\ref{prop:drestmamlest} and using the identity $\YY_j=\XX_j\trans\tasktheta+\ee_{j}$,
\begin{align*}
    \drest-\drsol &= (\XX\trans)^+\YY-\drsol \\
    &= (\XX\trans)^+\begin{bmatrix}\vdots \\ \XX_j\trans\tasktheta+\ee_{j} \\ \vdots\end{bmatrix}-\drsol \\
    &= (\XX\trans)^+\begin{bmatrix}\vdots \\  \XX_j\trans(\tasktheta-\drsol)+\ee_{j} \\ \vdots\end{bmatrix}+(\XX\trans)^+\begin{bmatrix}\vdots \\ \XX_j\trans\drsol \\ \vdots\end{bmatrix}-\drsol \\
    &= (\XX\XX\trans)^+\XX\begin{bmatrix}\vdots \\ \XX_j\trans(\tasktheta-\drsol)+\ee_{j} \\ \vdots\end{bmatrix}+(\XX\XX\trans)^+\XX\XX\trans\drsol-\drsol \\
    &= U(DD\trans)^+U\trans\sum_{j=1}^M\left(\XX_j\XX_j\trans(\tasktheta-\drsol)+\XX_j\ee_{j}\right) \\
    &\quad+U(DD\trans)^+(DD\trans)U\trans\drsol-\drsol
\end{align*}
Note that $DD\trans$ is a diagonal matrix of eigenvalues of $\XX\XX\trans$; $(DD\trans)^+$ is a diagonal matrix with entries the reciprocals of the nonzero eigenvalues of $\XX\XX\trans$ and the rest zeros.
Then, $(DD\trans)^+(DD\trans)$ is a diagonal matrix with $r$ ones, where $r$ is the number of nonzero eigenvalues of $\XX\XX\trans$, and $U(DD\trans)^+(DD\trans)U\trans=diag(I_r,0)$. 
Let $\lambda_{min}()$ denote the smallest eigenvalue of a matrix.
Thus,
\begin{align}\label{eq:normdiffdr}
    \begin{split}
    \norm{\drest-\drsol}_2 &\leq \lambda_{min}(\XX\XX\trans)^{-1}\norm{\sum_{j=1}^M(\XX_j\XX_j\trans(\tasktheta-\drsol)+\XX_j\ee_{j})} \\
    &\quad+\norm{\drsol}\mathbb{I}\{\lambda_{min}(\XX\XX\trans)=0\}
    \end{split}
\end{align}
where
\begin{align}\label{eq:xxtmineig}
    & \lambda_{min}(\XX\XX\trans) = \lambda_{min}\left(\sum_{j=1}^M\XX_j\XX_j\trans\right) \notag \\
    &= \lambda_{min}\left(2N\sum_{j=1}^M(\dfrac{\XX_j\XX_j\trans}{2N}-\QQ_j)+2N\sum_{j=1}^M (\QQ_j-\Ee_\gamma[\Qg])+2NM\Ee_\gamma[\Qg]\right) \notag \\
    &\geq 2NM\lambda_{min}(\Ee_\gamma[\Qg])+2N\lambda_{min}(\sum_{j=1}^M (\QQ_j-\Ee_\gamma[\Qg]))+2N\sum_{j=1}^M\lambda_{min}(\dfrac{\XX_j\XX_j\trans}{2N}-\QQ_j) \notag \\
    &\geq 2NM\lambda_{min}(\Ee_\gamma[\Qg])-2N\norm{\sum_{j=1}^M (\QQ_j-\Ee_\gamma[\Qg])}-2N\sum_{j=1}^M\norm{\dfrac{\XX_j\XX_j\trans}{2N}-\QQ_j},
\end{align}
{\small
\begin{align}\label{eq:xynormbound}
    \norm{\sum_{j=1}^M\XX_j(\XX_j\trans(\tasktheta-\drsol)+\ee_{j})} \notag 
    &= 2N\norm{\sum_{j=1}^M(\dfrac{\XX_j\XX_j\trans}{2N}-\QQ_j)(\tasktheta-\drsol)+\sum_{j=1}^M \QQ_j(\tasktheta-\drsol)+\sum_{j=1}^M\frac{\XX_j\ee_j}{2N}} \notag \\
    \begin{split}
    &\leq 2N\sum_{j=1}^M\norm{\dfrac{\XX_j\XX_j\trans}{2N}-\QQ_j}\norm{\tasktheta-\drsol}+2N\norm{\sum_{j=1}^M(\QQ_j\tasktheta-\Ee_\gamma[\Qg\Thetag])} \\
    &\quad+2N\norm{\sum_{j=1}^M(\QQ_j-\Ee_\gamma[\Qg])}\norm{\drsol}+\sum_{j=1}^M\norm{\XX_j\ee_j}.
    \end{split}
\end{align}}

Let $\omega>0$. Consider the following probabilistic events. Using union bound, at least one of them occurs with probability at most $2(2p+1+M+(p+1)M)e^{-\omega}$ 

\begin{itemize}[noitemsep,topsep=1pt,parsep=1pt,partopsep=1pt]
    \item (E1): $\norm{\sum_{j=1}^M(\QQ_j-\Ee_\gamma[\Qg])}\geq \dfrac{2\beta\omega}{3}+\sqrt{2M\norm{\var_\gamma[\Qg]}\omega}$, where $\norm{\Qg}\leq\beta$ with probability $1$.  This event occurs with probability at most $2pe^{-\omega}$, by Lemma~\ref{lem:qghpbound}.
    
    \item (E2): $\norm{\sum_{j=1}^M(\QQ_j\tasktheta-\Ee_\gamma[\Qg\Thetag])}\geq \dfrac{2\beta\eta\omega}{3}+\sqrt{2M\trace(\var_\gamma[\Qg\Thetag])\omega}$. Occurs with probability at most $2(p+1)e^{-\omega}$, by Lemma~\ref{lem:qgtghpbound}.
    
    \item (E3-1, $\dots$, E3-M): For $j=1,\dots,M$, $\norm{\dfrac{\XX_j\XX_j\trans}{2N}-\QQ_j}\geq \beta CK^2(\sqrt{\dfrac{p+\omega}{2N}}+\dfrac{p+\omega}{2N})$, where $\norm{\Qg}\leq \beta$ with probability $1$, the distribution of $\xx_{\gamma,i}$ conditional on $\gamma$ is sub-Gaussian with parameter $K$, and $C$ is a constant. For each $j$, this occurs with probability at most $2e^{-\omega}$, from extending Lemma~\ref{lem:covbound} to $\XX_j$.
    
    \item (E4-1, $\dots$, E4-M):
    For $j=1,\dots,M$, $\norm{\XX_j\ee_j}\geq\dfrac{2\xi\phi\omega}{3}+\sqrt{4N\trace(\Ee_\gamma[\sigmag\Qg])\omega}$, where $\norm{\xx_{\gamma,i}}\leq\xi$ and $\abs{\epsilon_{\gamma,i}}\leq\phi$ with probability $1$. For each $j$, this occurs with probability at most $2(p+1)e^{-\omega}$, from Lemma~\ref{lem:xgegbound} to $\XX_j\ee_j$.
\end{itemize}


From~\eqref{eq:xxtmineig} and~\eqref{eq:xynormbound}, with probability at least $1-2(pM+2M+2p+1)e^{-\omega}$,
{\small \begin{align*}
    \lambda_{min}(\XX\XX\trans) 
    &\geq 2NM\lambda_{min}(\Ee_\gamma[\Qg])-2N(\dfrac{2\beta\omega}{3}+\sqrt{2M\norm{\var_\gamma[\Qg]}\omega}+M(\beta CK^2(\sqrt{\dfrac{p+\omega}{2N}}+\dfrac{p+\omega}{2N})))) \\
    &= 2NM\left(\lambda_{min}(\Ee_\gamma[\Qg])-(\sqrt{\dfrac{2\norm{\var_\gamma[\Qg]}\omega}{M}}+\dfrac{2\beta\omega}{3M})-\beta CK^2(\sqrt{\dfrac{p+\omega}{2N}}+\dfrac{p+\omega}{2N})\right),
\end{align*}}
\begin{align*}
    &\norm{\sum_{j=1}^M(\XX_j\XX_j\trans(\tasktheta-\drsol)+\XX_j\ee_{j})} \\
    &\leq 2NM\tau\beta CK^2(\sqrt{\dfrac{p+\omega}{2N}}+\dfrac{p+\omega}{2N})+2N(\dfrac{2\beta\eta\omega}{3}+\sqrt{2M\trace(\var_\gamma[\Qg\Thetag])\omega}) \\
    &\quad+2N\norm{\drsol}(\dfrac{2\beta\omega}{3}+\sqrt{2M\norm{\var_\gamma[\Qg]}\omega})+M(\dfrac{2\xi\phi\omega}{3}+\sqrt{4N\trace(\Ee_\gamma[\sigmag\Qg])\omega}) \\
    &\leq 2NM\bigg(\tau\beta CK^2(\sqrt{\dfrac{p+\omega}{2N}}+\dfrac{p+\omega}{2N})+(\sqrt{\dfrac{2\trace(\var_\gamma[\Qg\Thetag])\omega}{M}}+\dfrac{2\beta\eta\omega}{3M}) \\
    &\quad\quad\quad\quad\quad+\norm{\drsol}(\sqrt{\dfrac{2\norm{\var_\gamma[\Qg]}\omega}{M}}+\dfrac{2\beta\omega}{3M})+(\sqrt{\dfrac{\trace(\Ee_\gamma[\sigmag\Qg])\omega}{N}}+\dfrac{\xi\phi\omega}{3N})\bigg).
\end{align*}
%where $\norm{\Thetag-\drsol}\leq\tau$ with probability $1$.

Thus, by~\eqref{eq:normdiffdr}, if $\lambda_{min}(\Ee_\gamma[\Qg])-(\sqrt{\dfrac{2\norm{\var_\gamma[\Qg]}\omega}{M}}+\dfrac{2\beta\omega}{3M})-\beta CK^2(\sqrt{\dfrac{p+\omega}{2N}}+\dfrac{p+\omega}{2N})>0$, with probability at least $1-2(pM+2M+2p+1)e^{-\omega}$, $\norm{\drest-\drsol}$ is bounded above by

\begin{equation*}
    \resizebox{\textwidth}{!}{$
    \dfrac{\tau\beta CK^2(\sqrt{\dfrac{p+\omega}{2N}}+\dfrac{p+\omega}{2N})+\sqrt{\dfrac{2\trace(\var_\gamma[\Qg\Thetag])\omega}{M}}+\dfrac{2\beta\eta\omega}{3M}+\norm{\drsol}(\sqrt{\dfrac{2\norm{\var_\gamma[\Qg]}\omega}{M}}+\dfrac{2\beta\omega}{3M})+\sqrt{\dfrac{\trace(\Ee_\gamma[\sigmag\Qg])\omega}{N}}+\dfrac{\xi\phi\omega}{3N}}{\lambda_{min}(\Ee_\gamma[\Qg])-(\sqrt{\dfrac{2\norm{\var_\gamma[\Qg]}\omega}{M}}+\dfrac{2\beta\omega}{3M})-\beta CK^2(\sqrt{\dfrac{p+\omega}{2N}}+\dfrac{p+\omega}{2N})}$}
\end{equation*}

Defining $\delta=2(pM+2M+2p+1)e^{-\omega}$, we let $\omega=\ln(pM+2M+2p+1)-\ln(\delta/2)$.
We have that $c_1(\omega,\norm{\var_\gamma[\Qg]},\trace(\var_\gamma[\Qg\Thetag]),\drsol)=\norm{\drsol}\sqrt{2\norm{\var_\gamma[\Qg]}\omega}+\sqrt{2\trace(\var_\gamma[\Qg\Thetag])\omega}$, $c_2(\omega)=\beta CK^2\sqrt{p+\omega}$, and $c_3(\omega)=\sqrt{\trace(\Ee_\gamma[\sigmag\Qg])\omega}$.

Hence, if $\lambda_{min}(\Ee_\gamma[\Qg])-\tilde{o}(1)>0$, with probability at least $1-\delta$, $\norm{\drest-\drsol}$ is bounded by
\begin{align*}
    &(\lambda_{min}(\Ee_\gamma[\Qg])-\tilde{o}(1))^{-1}(\dfrac{c_1(\omega,\norm{\var_\gamma[\Qg]},\trace(\var_\gamma[\Qg\Thetag]),\drsol)}{\sqrt{M}}+\dfrac{\tau}{\sqrt{2}}\dfrac{c_2(\omega)}{\sqrt{N}}+\dfrac{c_3(\omega)}{\sqrt{N}} \\
    &\hspace{4cm}+\tilde{o}(\dfrac{1}{\sqrt{M}})+\tilde{o}(\dfrac{1}{\sqrt{N}}))
\end{align*}
where $\omega=\ln(pM+2M+2p+1)-\ln(\delta/2)$.
\end{proof}

\subsubsection{Theorem~\ref{thm:mamlbound}}

\begin{proof}
Let $\ee_{j1}$ be the $N$-dimensional vector with entries $\epsilon_{j,i}, i=1,\dots,N$ and $\ee_{j2}$ be the $N$-dimensional vector with entries $\epsilon_{j,i}, i=N+1,\dots,2N$.
Let the SVD of $\WW$ be $UDV\trans$.
Then, from Proposition~\ref{prop:drestmamlest} and using the identities $\YY_{j1}=\XX_{j1}\trans\tasktheta+\ee_{j1}$ and $\YY_{j2}=\XX_{j2}\trans\tasktheta+\ee_{j2}$,
\begin{align*}
    &\mamlest-\mamlsol \\ &= (\WW\trans)^+\ZZ-\mamlsol \\
    &= (\WW\trans)^+\begin{bmatrix}\vdots \\ \XX_{j2}\trans\tasktheta+\ee_{j2}-\alpha\XX_{j2}\trans\XX_{j1}(\XX_{j1}\trans\tasktheta+\ee_{j1})/N \\ \vdots\end{bmatrix}-\mamlsol \\
    &= (\WW\trans)^+\begin{bmatrix}\vdots \\ \XX_{j2}\trans(\II-\dfrac{\alpha}{N}\XX_{j1}\XX_{j1}\trans)(\tasktheta-\mamlsol)+\ee_{j2}-\dfrac{\alpha}{N}\XX_{j2}\trans\XX_{j1}\ee_{j1} \\ \vdots\end{bmatrix} \\
    &\quad+(\WW\trans)^+\begin{bmatrix}\vdots \\ \XX_{j2}\trans(\II-\dfrac{\alpha}{N}\XX_{j1}\XX_{j1}\trans)\mamlsol \\ \vdots\end{bmatrix}-\mamlsol \\
    &= (\WW\WW\trans)^+\WW\begin{bmatrix}\vdots \\ \XX_{j2}\trans(\II-\dfrac{\alpha}{N}\XX_{j1}\XX_{j1}\trans)(\tasktheta-\mamlsol)+\ee_{j2}-\dfrac{\alpha}{N}\XX_{j2}\trans\XX_{j1}\ee_{j1} \\ \vdots\end{bmatrix} \\
    &\quad+(\WW\WW\trans)^+\WW\WW\trans\mamlsol-\mamlsol \\
    &= (UDD\trans U\trans)^+\sum_{j=1}^M((\II-\dfrac{\alpha}{N}\XX_{j1}\XX_{j1}\trans)\XX_{j2}\XX_{j2}\trans(\II-\dfrac{\alpha}{N}\XX_{j1}\XX_{j1}\trans)(\tasktheta-\mamlsol) \\
    &\hspace{3.2cm}+(\II-\dfrac{\alpha}{N}\XX_{j1}\XX_{j1}\trans)(\XX_{j2}\ee_{j2}-\dfrac{\alpha}{N}\XX_{j2}\XX_{j2}\trans\XX_{j1}\ee_{j1})) \\
    &\quad+(UDD\trans U\trans)^+UDD\trans U\trans\mamlsol-\mamlsol
\end{align*}


Note that $DD\trans$ is a diagonal matrix of eigenvalues of $\WW\WW\trans$; $(DD\trans)^+$ is a diagonal matrix with entries the reciprocals of the nonzero eigenvalues of $\WW\WW\trans$ and the rest zeros.
Then, $(DD\trans)^+(DD\trans)$ is a diagonal matrix with $r$ ones, where $r$ is the number of nonzero eigenvalues of $\WW\WW\trans$, and $U(DD\trans)^+(DD\trans)U\trans=diag(I_r,0)$. 
Let $\lambda_{min}()$ denote the smallest eigenvalue of a matrix.
Thus,
\begin{align}\label{eq:normdiffmaml}
    \begin{split}
    &\norm{\mamlest-\mamlsol}  \\
    &\leq \lambda_{min}(\WW\WW\trans)^{-1}\bigg\lVert\sum_{j=1}^M((\II-\dfrac{\alpha}{N}\XX_{j1}\XX_{j1}\trans)\XX_{j2}\XX_{j2}\trans(\II-\dfrac{\alpha}{N}\XX_{j1}\XX_{j1}\trans)(\tasktheta-\mamlsol) \\
    &\hspace{3cm}+(\II-\dfrac{\alpha}{N}\XX_{j1}\XX_{j1}\trans)(\XX_{j2}\ee_{j2}-\dfrac{\alpha}{N}\XX_{j2}\XX_{j2}\trans\XX_{j1}\ee_{j1}))\bigg\rVert\\
    &\quad+\norm{\mamlsol}\mathbb{I}\{\lambda_{min}(\WW\WW\trans)=0\}
    \end{split}
\end{align}
where

\begin{equation}
\begin{aligned}\label{eq:wwtmineig}
    & \lambda_{min}(\WW\WW\trans)  \\
    &= \lambda_{min}\left(\sum_{j=1}^M(\II-\dfrac{\alpha}{N}\XX_{j1}\XX_{j1}\trans)\XX_{j2}\XX_{j2}\trans(\II-\dfrac{\alpha}{N}\XX_{j1}\XX_{j1}\trans)\right) \notag \\
    &\geq\lambda_{min}\bigg(N\sum_{j=1}^M(\II-\alpha \QQ_j)\QQ_j(\II-\alpha \QQ_j)-N\alpha\sum_{j=1}^M(\II-\alpha \QQ_j)\QQ_j(\dfrac{\XX_{j1}\XX_{j1}\trans}{N}-\QQ_j) \notag \\
    &\quad-N\alpha\sum_{j=1}^M(\dfrac{\XX_{j1}\XX_{j1}\trans}{N}-\QQ_j)\QQ_j(\II-\alpha \QQ_j)+N\sum_{j=1}^M(\II-\alpha \QQ_j)(\dfrac{\XX_{j2}\XX_{j2}\trans}{N}-\QQ_j)(\II-\alpha \QQ_j) \notag \\
    &\quad-N\alpha\sum_{j=1}^M(\II-\alpha \QQ_j)(\dfrac{\XX_{j2}\XX_{j2}\trans}{N}-\QQ_j)(\dfrac{\XX_{j1}\XX_{j1}\trans}{N}-\QQ_j) \notag  \\
    &\quad-N\alpha\sum_{j=1}^M(\dfrac{\XX_{j1}\XX_{j1}\trans}{N}-\QQ_j)(\dfrac{\XX_{j2}\XX_{j2}\trans}{N}-\QQ_j)(\II-\alpha \QQ_j) \notag \\
    &\quad+N\alpha^2\sum_{j=1}^M(\dfrac{\XX_{j1}\XX_{j1}\trans}{N}-\QQ_j)\dfrac{\XX_{j2}\XX_{j2}\trans}{N}(\dfrac{\XX_{j1}\XX_{j1}\trans}{N}-\QQ_j) \bigg)\notag \\
    &\geq MN\lambda_{min}(\Ee_\gamma[(\II-\alpha\Qg)\Qg(\II-\alpha\Qg)]) \\
    &\quad-N\norm{\sum_{j=1}^M((\II-\alpha \QQ_j)\QQ_j(\II-\alpha \QQ_j)-\Ee_\gamma[(\II-\alpha\Qg)\Qg(\II-\alpha\Qg)])} \\
    &\quad-2N\alpha\sum_{j=1}^M\norm{\II-\alpha \QQ_j}\norm{\QQ_j}\norm{\dfrac{\XX_{j1}\XX_{j1}\trans}{N}-\QQ_j} \\
    &\quad-N\sum_{j=1}^M\norm{\II-\alpha \QQ_j}^2\norm{\dfrac{\XX_{j2}\XX_{j2}\trans}{N}-\QQ_j} \\
    &\quad-2N\alpha\sum_{j=1}^M\norm{\II-\alpha \QQ_j}\norm{\dfrac{\XX_{j1}\XX_{j1}\trans}{N}-\QQ_j}\norm{\dfrac{\XX_{j2}\XX_{j2}\trans}{N}-\QQ_j}
\end{aligned}
\end{equation}


and
\begin{align}\label{eq:wznormbound}
    &\bigg\lVert\sum_{j=1}^M((\II-\dfrac{\alpha}{N}\XX_{j1}\XX_{j1}\trans)\XX_{j2}\XX_{j2}\trans(\II-\dfrac{\alpha}{N}\XX_{j1}\XX_{j1}\trans)(\tasktheta-\mamlsol) \notag \\
    &\quad\quad\quad+(\II-\dfrac{\alpha}{N}\XX_{j1}\XX_{j1}\trans)(\XX_{j2}\ee_{j2}-\dfrac{\alpha}{N}\XX_{j2}\XX_{j2}\trans\XX_{j1}\ee_{j1}))\bigg\rVert \notag \\
    \iffalse
    &=\bigg\lVert N\sum_{j=1}^M((\II-\dfrac{\alpha}{N}\XX_{j1}\XX_{j1}\trans)\dfrac{\XX_{j2}\XX_{j2}\trans}{N}(\II-\dfrac{\alpha}{N}\XX_{j1}\XX_{j1}\trans)-(\II-\alpha \QQ_j)\QQ_j(\II-\alpha \QQ_j))(\tasktheta-\mamlsol) \notag \\
    &\quad\quad+N\sum_{j=1}^M((\II-\alpha \QQ_j)\QQ_j(\II-\alpha \QQ_j)\tasktheta-\Ee_\gamma[(\II-\alpha\Qg)\Qg(\II-\alpha\Qg)\Thetag]) \notag \\
    &\quad\quad-N\sum_{j=1}^M((\II-\alpha \QQ_j)\QQ_j(\II-\alpha \QQ_j)-\Ee_\gamma[(\II-\alpha\Qg)\Qg(\II-\alpha\Qg)])\mamlsol \notag \\
    &\quad\quad+\sum_{j=1}^M(\II-\alpha \QQ_j)(\XX_{j2}\ee_{j2}-(\dfrac{\alpha}{N}\XX_{j2}\XX_{j2}\trans-\alpha \QQ_j+\alpha \QQ_j)\XX_{j1}\ee_{j1}) \notag \\
    &\quad\quad-\alpha\sum_{j=1}^M(\dfrac{\XX_{j1}\XX_{j1}\trans}{N}-\QQ_j)(\XX_{j2}\ee_{j2}-(\dfrac{\alpha}{N}\XX_{j2}\XX_{j2}\trans-\alpha \QQ_j+\alpha \QQ_j)\XX_{j1}\ee_{j1})\bigg\rVert \notag \\
    \fi
    \begin{split}
    &\leq N\norm{\sum_{j=1}^M((\II-\alpha \QQ_j)\QQ_j(\II-\alpha \QQ_j)\tasktheta-\Ee_\gamma[(\II-\alpha\Qg)\Qg(\II-\alpha\Qg)\Thetag])} \\
    &\quad+N\norm{\sum_{j=1}^M((\II-\alpha \QQ_j)\QQ_j(\II-\alpha \QQ_j)-\Ee_\gamma[(\II-\alpha\Qg)\Qg(\II-\alpha\Qg)])}\norm{\mamlsol} \\
    &\quad+2N\alpha\sum_{j=1}^M\norm{\II-\alpha \QQ_j}\norm{\QQ_j}\norm{\dfrac{\XX_{j1}\XX_{j1}\trans}{N}-\QQ_j}\norm{\tasktheta-\mamlsol} \\
    &\quad+N\sum_{j=1}^M\norm{\II-\alpha \QQ_j}^2\norm{\dfrac{\XX_{j2}\XX_{j2}\trans}{N}-\QQ_j}\norm{\tasktheta-\mamlsol}  \\
    &\quad+2N\alpha\sum_{j=1}^M\norm{\II-\alpha \QQ_j}\norm{\dfrac{\XX_{j1}\XX_{j1}\trans}{N}-\QQ_j}\norm{\dfrac{\XX_{j2}\XX_{j2}\trans}{N}-\QQ_j}\norm{\tasktheta-\mamlsol} \\
    &\quad+N\alpha^2\sum_{j=1}^M\norm{\QQ_j}\norm{\dfrac{\XX_{j1}\XX_{j1}\trans}{N}-\QQ_j}^2\norm{\tasktheta-\mamlsol} \\
    &\quad+N\alpha^2\sum_{j=1}^M\norm{\dfrac{\XX_{j1}\XX_{j1}\trans}{N}-\QQ_j}^2\norm{\dfrac{\XX_{j2}\XX_{j2}\trans}{N}-\QQ_j}\norm{\tasktheta-\mamlsol} \\
    &\quad+\sum_{j=1}^M\norm{\II-\alpha \QQ_j}\norm{\XX_{j2}\ee_{j2}}+\alpha\sum_{j=1}^M\norm{\II-\alpha \QQ_j}\norm{\dfrac{\XX_{j2}\XX_{j2}\trans}{N}-\QQ_j}\norm{\XX_{j1}\ee_{j1}} \\
    &\quad+\alpha\sum_{j=1}^M\norm{\II-\alpha \QQ_j}\norm{\QQ_j}\norm{\XX_{j1}\ee_{j1}}+\alpha\sum_{j=1}^M\norm{\dfrac{\XX_{j1}\XX_{j1}\trans}{N}-\QQ_j}\norm{\XX_{j2}\ee_{j2}} \\
    &\quad+\alpha^2\sum_{j=1}^M\norm{\dfrac{\XX_{j1}\XX_{j1}\trans}{N}-\QQ_j}\norm{\dfrac{\XX_{j2}\XX_{j2}\trans}{N}-\QQ_j}\norm{\XX_{j1}\ee_{j1}} 
    +\alpha^2\sum_{j=1}^M\norm{\dfrac{\XX_{j1}\XX_{j1}\trans}{N}-\QQ_j}\norm{\QQ_j}\norm{\XX_{j1}\ee_{j1}}
    \end{split}
\end{align}

Let $\omega>0$. Consider the following probabilistic events:
\begin{itemize}
    \item (E1): $\norm{\sum_{j=1}^M((\II-\alpha \QQ_j)\QQ_j(\II-\alpha \QQ_j)-\Ee_\gamma[(\II-\alpha\Qg)\Qg(\II-\alpha\Qg)])}\geq\dfrac{2\beta\mu^2\omega}{3}+\sqrt{2M\norm{\var_\gamma[\SSS_\gamma]}\omega}$, where $\norm{\Qg}\leq\beta$ and $\norm{\II-\alpha\Qg}\leq\mu$ with probability $1$.
    
    This occurs with probability at most $2pe^{-\omega}$, from the remark after Lemma~\ref{lem:qghpbound}.
    
    \item (E2): $\norm{\sum_{j=1}^M((\II-\alpha \QQ_j)\QQ_j(\II-\alpha \QQ_j)\tasktheta-\Ee_\gamma[(\II-\alpha\Qg)\Qg(\II-\alpha\Qg)\Thetag])}\geq\dfrac{2\beta\mu^2\eta\omega}{3}+\sqrt{2M\trace(\var_\gamma[\SSS_\gamma\Thetag])\omega}$ where $\norm{\Qg}\leq\beta$, $\norm{\II-\alpha\Qg}\leq\mu$, and $\norm{\Thetag}\leq\eta$ with probability $1$.
    
    This occurs with probability at most $2(p+1)e^{-\omega}$, from the remark after Lemma~\ref{lem:qgtghpbound}.
    
    \item (E3-1, $\dots$, E3-2M): For $j=1,\dots,M$, $\norm{\dfrac{\XX_{j1}\XX_{j1}\trans}{N}-\QQ_j}\geq \beta CK^2(\sqrt{\dfrac{p+\omega}{N}}+\dfrac{p+\omega}{N})$ and $\norm{\dfrac{\XX_{j2}\XX_{j2}\trans}{N}-\QQ_j}\geq \beta CK^2(\sqrt{\dfrac{p+\omega}{N}}+\dfrac{p+\omega}{N})$, where $\norm{\Qg}\leq \beta$ with probability $1$, the distribution of $\xx_{\gamma,i}$ conditional on $\gamma$ is sub-Gaussian with parameter $K$, and $C$ is a constant.
    
    Each of the $2M$ events occurs with probability at most $2e^{-\omega}$, from Lemma~\ref{lem:covbound}.
    
    \item (E4-1, $\dots$, E4-2M):
    For $j=1,\dots,M$, $\norm{\XX_{j1}\ee_{j1}}\geq\dfrac{2\xi\phi\omega}{3}+\sqrt{2N\trace(\Ee_\gamma[\sigmag\Qg])\omega}$ and $\norm{\XX_{j2}\ee_{j2}}\geq\dfrac{2\xi\phi\omega}{3}+\sqrt{2N\trace(\Ee_\gamma[\sigmag\Qg])\omega}$, where $\norm{\xx_{\gamma,i}}\leq\xi$ and $\abs{\epsilon_{\gamma,i}}\leq\phi$ with probability $1$.
    
    Each of the $2M$ events occurs with probability at most $2(p+1)e^{-\omega}$, from Lemma~\ref{lem:xgegbound}.
\end{itemize}
From the union bound, at least one of the events (E1), (E2), (E3-1), $\dots$, (E3-2M), (E4-1), $\dots$, (E4-2M) occurs with probability at most $2(2p+1+2M+2M(p+1))e^{-\omega}$.
That is, none of the events occur with probability at least $1-2(2pM+4M+2p+1)e^{-\omega}$.

From~\eqref{eq:wwtmineig} and~\eqref{eq:wznormbound}, with probability at least $1-2(2pM+4M+2p+1)e^{-\omega}$,
\begin{align*}
    &\lambda_{min}(\WW\WW\trans) \\
    &\geq MN\lambda_{min}(\Ee_\gamma[(\II-\alpha\Qg)\Qg(\II-\alpha\Qg)])-N(\dfrac{2\beta\mu^2\omega}{3}+\sqrt{2M\norm{\var_\gamma[\SSS_\gamma]}\omega}) \\
    &\quad-2\alpha MN\beta^2\mu CK^2(\sqrt{\dfrac{p+\omega}{N}}+\dfrac{p+\omega}{N})-MN\beta\mu^2CK^2(\sqrt{\dfrac{p+\omega}{N}}+\dfrac{p+\omega}{N}) \\
    &\quad-2\alpha MN\beta^2\mu C^2K^4(\sqrt{\dfrac{p+\omega}{N}}+\dfrac{p+\omega}{N})^2 \\
    &=MN\bigg(\lambda_{min}(\Ee_\gamma[\SSS_\gamma])-(\sqrt{\dfrac{2\norm{\var_\gamma[\SSS_\gamma]}\omega}{M}}+\dfrac{2\beta\mu^2\omega}{3M}) \\
    &\quad\quad\quad\quad-(2\alpha\beta^2\mu +\beta\mu^2)CK^2(\sqrt{\dfrac{p+\omega}{N}}+\dfrac{p+\omega}{N})-2\alpha\beta^2\mu C^2K^4(\sqrt{\dfrac{p+\omega}{N}}+\dfrac{p+\omega}{N})^2\bigg)
\end{align*}
and
\begin{align*}
    &\lVert\sum_{j=1}^M((\II-\dfrac{\alpha}{N}\XX_{j1}\XX_{j1}\trans)\XX_{j2}\XX_{j2}\trans(\II-\dfrac{\alpha}{N}\XX_{j1}\XX_{j1}\trans)(\tasktheta-\mamlsol) \notag \\
    &\quad\quad\quad+(\II-\dfrac{\alpha}{N}\XX_{j1}\XX_{j1}\trans)(\XX_{j2}\ee_{j2}-\dfrac{\alpha}{N}\XX_{j2}\XX_{j2}\trans\XX_{j1}\ee_{j1}))\bigg\rVert \\
    \iffalse
    &\leq N(\dfrac{2\beta\mu^2\eta\omega}{3}+\sqrt{2M\trace(\var_\gamma[\SSS_\gamma\Thetag])\omega})+N(\dfrac{2\beta\mu^2\omega}{3}+\sqrt{2M\norm{\var_\gamma[\SSS_\gamma]}\omega})\norm{\mamlsol} \\
    &\quad+2\alpha MN\tau'\beta^2\mu CK^2(\sqrt{\dfrac{p+\omega}{N}}+\dfrac{p+\omega}{N})+MN\tau'\beta\mu^2 CK^2(\sqrt{\dfrac{p+\omega}{N}}+\dfrac{p+\omega}{N}) \\
    &\quad+2\alpha MN\tau'\beta^2\mu C^2K^4(\sqrt{\dfrac{p+\omega}{N}}+\dfrac{p+\omega}{N})^2+\alpha^2 MN\tau'\beta^3C^2K^4(\sqrt{\dfrac{p+\omega}{N}}+\dfrac{p+\omega}{N})^2 \\
    &\quad+\alpha^2 MN\tau'\beta^3C^3K^6(\sqrt{\dfrac{p+\omega}{N}}+\dfrac{p+\omega}{N})^3+M\mu(\dfrac{2\xi\phi\omega}{3}+\sqrt{2N\trace(\Ee_\gamma[\sigmag\Qg])\omega}) \\
    &\quad+\alpha M\beta\mu CK^2(\sqrt{\dfrac{p+\omega}{N}}+\dfrac{p+\omega}{N})(\dfrac{2\xi\phi\omega}{3}+\sqrt{2N\trace(\Ee_\gamma[\sigmag\Qg])\omega}) \\
    &\quad+\alpha M\beta\mu(\dfrac{2\xi\phi\omega}{3}+\sqrt{2N\trace(\Ee_\gamma[\sigmag\Qg])\omega}) \\
    &\quad+\alpha M\beta CK^2(\sqrt{\dfrac{p+\omega}{N}}+\dfrac{p+\omega}{N})(\dfrac{2\xi\phi\omega}{3}+\sqrt{2N\trace(\Ee_\gamma[\sigmag\Qg])\omega}) \\
    &\quad+\alpha^2 M\beta^2C^2K^4(\sqrt{\dfrac{p+\omega}{N}}+\dfrac{p+\omega}{N})^2(\dfrac{2\xi\phi\omega}{3}+\sqrt{2N\trace(\Ee_\gamma[\sigmag\Qg])\omega}) \\
    &\quad+\alpha^2 M\beta^2CK^2(\sqrt{\dfrac{p+\omega}{N}}+\dfrac{p+\omega}{N})(\dfrac{2\xi\phi\omega}{3}+\sqrt{2N\trace(\Ee_\gamma[\sigmag\Qg])\omega}) \\
    \fi
    &\leq MN\bigg((\sqrt{\dfrac{2\trace(\var_\gamma[\SSS_\gamma\Thetag])\omega}{M}}+\dfrac{2\beta\mu^2\eta\omega}{3M})+\norm{\mamlsol}(\sqrt{\dfrac{2\norm{\var_\gamma[\SSS_\gamma]}\omega}{M}}+\dfrac{2\beta\mu^2\omega}{3M}) \\
    &\quad\quad\quad\quad+(2\alpha\beta+\mu)\tau'\beta\mu CK^2(\sqrt{\dfrac{p+\omega}{N}}+\dfrac{p+\omega}{N})+(2\mu+\alpha\beta)\alpha\tau'\beta^2C^2K^4(\sqrt{\dfrac{p+\omega}{N}})^2 \\
    &\quad\quad\quad\quad+(1+\alpha\beta)\mu(\sqrt{\dfrac{2\trace(\Ee_\gamma[\sigmag\Qg])\omega}{N}}+\dfrac{2\xi\phi\omega}{3N}) \\
    &\quad\quad\quad\quad+(\mu+1+\alpha\beta)\alpha\beta CK^2\sqrt{\dfrac{p+\omega}{N}}\sqrt{\dfrac{2\trace(\Ee_\gamma[\sigmag\Qg])\omega}{N}}+o(\dfrac{1}{N})\bigg)
\end{align*}
where $\norm{\Thetag-\mamlsol}\leq\tau'$ with probability $1$.

Thus, by~\eqref{eq:normdiffmaml}, if 
\begin{align*}
    &\lambda_{min}(\Ee_\gamma[\SSS_\gamma])-(\sqrt{\dfrac{2\norm{\var_\gamma[\SSS_\gamma]}\omega}{M}}+\dfrac{2\beta\mu^2\omega}{3M}) \\
    &\quad\quad-(2\alpha\beta^2\mu +\beta\mu^2)CK^2(\sqrt{\dfrac{p+\omega}{N}}+\dfrac{p+\omega}{N})-2\alpha\beta^2\mu C^2K^4(\sqrt{\dfrac{p+\omega}{N}}+\dfrac{p+\omega}{N})^2>0,
\end{align*} 
with probability at least $1-2(2pM+4M+2p+1)e^{-\omega}$, $\norm{\mamlest-\mamlsol}$ is bounded above by
\begin{align*}
    &(\lambda_{min}(\Ee_\gamma[\SSS_\gamma])-o(1))^{-1}\bigg(\sqrt{\dfrac{2\trace(\var_\gamma[\SSS_\gamma\Thetag])\omega}{M}}+\norm{\mamlsol}\sqrt{\dfrac{2\norm{\var_\gamma[\SSS_\gamma]}\omega}{M}} \\
    &\quad+(2\alpha\beta+\mu)\tau'\beta\mu CK^2\sqrt{\dfrac{p+\omega}{N}}+(1+\alpha\beta)\mu\sqrt{\dfrac{2\trace(\Ee_\gamma[\sigmag\Qg])\omega}{N}}+\dfrac{2\beta\mu^2\eta\omega}{3M} \\
    &\quad+\norm{\mamlsol}\dfrac{2\beta\mu^2\omega}{3M}+((2\alpha\beta+\mu)\mu+(2\mu+\alpha\beta)\alpha\beta CK^2)\tau'\beta CK^2\dfrac{p+\omega}{N} \\
    &\quad+(1+\alpha\beta)\mu\dfrac{2\xi\phi\omega}{3N}+(\mu+1+\alpha+\beta)\alpha\beta CK^2\dfrac{\sqrt{p+\omega}\sqrt{2\trace(\Ee_\gamma[\sigmag\Qg])\omega}}{N}+o(\dfrac{1}{N})\bigg)
\end{align*}

Setting $\delta=2(2pM+4M+2p+1)e^{-\omega}$, we obtain $\omega=\ln(2pM+4M+2p+1)-\ln(\delta/2)$.

Thus, if $\lambda_{min}(\Ee_\gamma[\SSS_\gamma])-\tilde{o}(1)>0$, with probability at least $1-\delta$, $\norm{\mamlest-\mamlsol}$ is bounded above by
\begin{align*}
    &(\lambda_{min}(\Ee_\gamma[\SSS_\gamma])-\tilde{o}(1))^{-1}\bigg(\dfrac{c_1(\omega,\norm{\var_\gamma[\SSS_\gamma]},\trace(\var_\gamma[\SSS_\gamma\Thetag]),\mamlsol)}{\sqrt{M}} \\
    &\hspace{3.5cm}+\dfrac{(2\alpha\beta+\mu)\mu\tau'c_2(\omega)+\sqrt{2}(1+\alpha\beta)\mu c_3(\omega)}{\sqrt{N}}+\tilde{o}(\dfrac{1}{\sqrt{M}})+\tilde{o}(\dfrac{1}{\sqrt{N}})\bigg)
\end{align*}

Note that $\norm{
\II-\alpha\Qg}\leq 1+\alpha\beta$, so we can replace $\mu$ in the above bound by $1+\alpha\beta$ to get the desired result.

\end{proof}

\subsection{Theorem~\ref{thm:loss}}

The precise form of the losses are as follows.
For arbitrary $\theta$,
\begin{align*}
    \Ee_\gamma[\lossgt] &= \dfrac12\btheta\trans\Ee_\gamma[\Qg]\btheta-\Ee_\gamma[\Qg\Thetag]\trans\btheta+\dfrac12\Ee_\gamma[\Thetag\trans\Qg\Thetag]+\dfrac12\Ee_\gamma[\sigmag] \\
    \Ee_\gamma[\Ee_{\oO_\gamma}[\rR(\tilde{\btheta}_\gamma(\alpha);\gamma)]] &= \dfrac12\btheta\trans\Ee_\gamma[\Ag]\btheta-\Ee_\gamma[\Ag\Thetag]\trans\btheta+\dfrac12\Ee_\gamma[\Thetag\trans\Ag\Thetag] \\
    &\quad+\dfrac12\Ee_\gamma[\sigmag]+\dfrac12\dfrac{\alpha^2}{N}\Ee_\gamma[\sigmag \trace(\Qg^2)] \\
    \text{where}\quad\Ag &= (\II-\alpha\Qg)\Qg(\II-\alpha\Qg)+\dfrac{\alpha^2}{N}(\Ee[\xx_{\gamma,i}\xx_{\gamma,i}\trans\Qg \xx_{\gamma,i}\xx_{\gamma,i}\trans]-\Qg^3)
\end{align*}

\begin{proof}
The result for $\Ee_\gamma[\lossgt]$ follows from the proof of Equation~\ref{eq:drmamlsols}.
$\Ee_\gamma[\lossgt]$ is minimized by $\drsol$ by definition.

Let $\XX_\gamma$ be the $p\times N$ matrix with columns $\xx_{\gamma,i}$ and $\YY_\gamma$ be the $N$-dimensional vector with entries $y_{\gamma,i}$. 
Recalling the definition of $\tilde{\btheta}_\gamma(\alpha)$, from~\eqref{eq:lossfunc}
\begin{align*}
    \rR(\tilde{\btheta}_\gamma(\alpha);\gamma) &= \rR(\btheta-\dfrac{\alpha}{N}(\XX_\gamma\XX_\gamma\trans\btheta-\XX_\gamma\YY_\gamma);\gamma) = \rR((\II-\dfrac{\alpha}{N}\XX_\gamma\XX_\gamma\trans)\btheta+\dfrac{\alpha}{N}\XX_\gamma\YY_\gamma);\gamma) \\
    &= \dfrac12((\II-\dfrac{\alpha}{N}\XX_\gamma\XX_\gamma\trans)\btheta+\dfrac{\alpha}{N}\XX_\gamma\YY_\gamma))\trans\Qg((\II-\dfrac{\alpha}{N}\XX_\gamma\XX_\gamma\trans)\btheta+\dfrac{\alpha}{N}\XX_\gamma\YY_\gamma))\\
    &\quad-\Thetag\trans\Qg((\II-\dfrac{\alpha}{N}\XX_\gamma\XX_\gamma\trans)\btheta+\dfrac{\alpha}{N}\XX_\gamma\YY_\gamma))+\dfrac12\Thetag\trans\Qg\Thetag+\dfrac12\sigmag \\
    &=\dfrac12\btheta\trans(\II-\dfrac{\alpha}{N}\XX_\gamma\XX_\gamma\trans)\Qg(\II-\dfrac{\alpha}{N}\XX_\gamma\XX_\gamma\trans)\btheta+\btheta\trans(\II-\dfrac{\alpha}{N}\XX_\gamma\XX_\gamma\trans)\Qg\dfrac{\alpha}{N}\XX_\gamma\YY_\gamma \\
    &\quad+\dfrac12\dfrac{\alpha^2}{N^2}\YY_\gamma\trans\XX_\gamma\trans\Qg\XX_\gamma\YY_\gamma-\Thetag\trans\Qg(\II-\dfrac{\alpha}{N}\XX_\gamma\XX_\gamma\trans)\btheta-\dfrac{\alpha}{N}\Thetag\trans\Qg\XX_\gamma\YY_\gamma \\
    &\quad+\dfrac12\Thetag\trans\Qg\Thetag+\dfrac12\sigmag
\end{align*}

First take the expectation with respect to $\YY_\gamma$.
Let $\ee_\gamma$ be the $N$-dimensional vector with entries $\epsilon_{\gamma,i}$.
\begin{align*}
    \Ee_{\YY_\gamma}[\rR(\tilde{\btheta}_\gamma(\alpha);\gamma)] &= \dfrac12\btheta\trans(\II-\dfrac{\alpha}{N}\XX_\gamma\XX_\gamma\trans)\Qg(\II-\dfrac{\alpha}{N}\XX_\gamma\XX_\gamma\trans)\btheta+\btheta\trans(\II-\dfrac{\alpha}{N}\XX_\gamma\XX_\gamma\trans)\Qg\dfrac{\alpha}{N}\XX_\gamma\XX_\gamma\trans\Thetag \\
    &\quad+\dfrac12\dfrac{\alpha^2}{N^2}\Ee_{\ee_\gamma}[(\Thetag\trans\XX_\gamma\XX_\gamma\trans+\ee_\gamma\trans\XX_\gamma\trans)\Qg(\XX_\gamma\XX_\gamma\trans\Thetag+\XX_\gamma\ee_\gamma)] \\
    &\quad-\Thetag\trans\Qg(\II-\dfrac{\alpha}{N}\XX_\gamma\XX_\gamma\trans)\btheta-\dfrac{\alpha}{N}\Thetag\trans\Qg\XX_\gamma\XX_\gamma\trans\Thetag+\dfrac12\Thetag\trans\Qg\Thetag+\dfrac12\sigmag \\
    &=\dfrac12\btheta\trans(\II-\dfrac{\alpha}{N}\XX_\gamma\XX_\gamma\trans)\Qg(\II-\dfrac{\alpha}{N}\XX_\gamma\XX_\gamma\trans)\btheta \\
    &\quad-\btheta\trans(\II-\dfrac{\alpha}{N}\XX_\gamma\XX_\gamma\trans)\Qg(\II-\dfrac{\alpha}{N}\XX_\gamma\XX_\gamma\trans)\Thetag \\
    &\quad+\dfrac12\Thetag\trans(\II-\dfrac{\alpha}{N}\XX_\gamma\XX_\gamma\trans)\Qg(\II-\dfrac{\alpha}{N}\XX_\gamma\XX_\gamma\trans)\Thetag+\dfrac12\sigmag+\dfrac12\dfrac{\alpha^2}{N^2}\sigmag \trace(\XX_\gamma\XX_\gamma\trans\Qg)
\end{align*}

Using the linearity of trace and expectation, as well as the cyclic property of trace,
\begin{align*}
    \Ee_{\ee_\gamma}[\ee_\gamma\trans\XX_\gamma\trans\Qg\XX_\gamma\ee_\gamma] &= \Ee_{\ee_\gamma}[\trace(\XX_\gamma\trans\Qg\XX_\gamma\ee_\gamma\ee_\gamma\trans)] = \trace(\XX_\gamma\trans\Qg\XX_\gamma\Ee_{\ee_\gamma}[\ee_\gamma\ee_\gamma\trans]) %\\
    %&= \trace(\XX_\gamma\trans\Qg\XX_\gamma\sigmag \II) 
    = \sigmag \trace(\XX_\gamma\XX_\gamma\trans\Qg)
\end{align*}

Using the previous equality,
\begin{align*}
    &\Ee_{\oO_\gamma}[\rR(\tilde{\btheta}_\gamma(\alpha);\gamma)] = \Ee_{\XX_\gamma}[\Ee_{\YY_\gamma}[\rR(\tilde{\btheta}_\gamma(\alpha);\gamma)]] \\
    &= \dfrac12\btheta\trans\Ee_{\XX_\gamma}[(\II-\dfrac{\alpha}{N}\XX_\gamma\XX_\gamma\trans)\Qg(\II-\dfrac{\alpha}{N}\XX_\gamma\XX_\gamma\trans)]\btheta 
    -\btheta\trans\Ee_{\XX_\gamma}[(\II-\dfrac{\alpha}{N}\XX_\gamma\XX_\gamma\trans)\Qg(\II-\dfrac{\alpha}{N}\XX_\gamma\XX_\gamma\trans)]\Thetag \\
    &\quad+\dfrac12\Thetag\trans\Ee_{\XX_\gamma}[(\II-\dfrac{\alpha}{N}\XX_\gamma\XX_\gamma\trans)\Qg(\II-\dfrac{\alpha}{N}\XX_\gamma\XX_\gamma\trans)]\Thetag 
    +\dfrac12\sigmag+\dfrac12\dfrac{\alpha^2}{N^2}\sigmag\Ee_{\XX_\gamma}[\trace(\XX_\gamma\XX_\gamma\trans\Qg)]
\end{align*}

We compute
\begin{align*}
    &\Ee_{\XX_\gamma}[(\II-\dfrac{\alpha}{N}\XX_\gamma\XX_\gamma\trans)\Qg(\II-\dfrac{\alpha}{N}\XX_\gamma\XX_\gamma\trans)] \\
    &=\Qg-2\alpha\Qg^2+\dfrac{\alpha^2}{N^2}\Ee_{\XX_\gamma}[\sum_{i=1}^N\sum_{j=1}^N \xx_{\gamma,i}\xx_{\gamma,i}\trans\Qg \xx_{\gamma,j}\xx_{\gamma,j}\trans] \\
    &=\Qg-2\alpha\Qg^2+\dfrac{\alpha^2}{N^2}\left(N^2\Qg^3+\sum_{i=1}^N(\Ee_{\xx_{\gamma,i}}[\xx_{\gamma,i}\xx_{\gamma,i}\trans\Qg \xx_{\gamma,i}\xx_{\gamma,i}\trans]-\Qg^3)\right) \\
    &= (\II-\alpha\Qg)\Qg(\II-\alpha\Qg)+\dfrac{\alpha^2}{N}(\Ee_{\xx_{\gamma,i}}[\xx_{\gamma,i}\xx_{\gamma,i}\trans\Qg \xx_{\gamma,i}\xx_{\gamma,i}\trans]-\Qg^3) \equiv \Ag
\end{align*}
and
\begin{align*}
    \Ee_{\XX_\gamma}[\trace(\XX_\gamma\XX_\gamma\trans\Qg)] &= \trace(\Ee_{\XX_\gamma}[\XX_\gamma\XX_\gamma\trans]\Qg) = N \trace(\Qg^2)
\end{align*}

Combining the previous two expressions,
\begin{align*}
    \Ee_{\oO_\gamma}[\rR(\tilde{\btheta}_\gamma(\alpha);\gamma)] &=\dfrac12\btheta\trans\Ag\btheta-\btheta\trans\Ag\Thetag+\dfrac12\Thetag\trans\Ag\Thetag+\dfrac12\sigmag+\dfrac12\dfrac{\alpha^2}{N}\sigmag \trace(\Qg^2)
\end{align*}
Taking the expectation with respect to $\gamma$ gives
\begin{align*}
    \Ee_\gamma[\Ee_{\oO_\gamma}[\rR(\tilde{\btheta}_\gamma(\alpha);\gamma)]] &=\dfrac12\btheta\trans\Ee_\gamma[\Ag]\btheta-\btheta\trans\Ee_\gamma[\Ag\Thetag]+\dfrac12\Ee_\gamma[\Thetag\trans\Ag\Thetag] \\
    &\quad+\dfrac12\sigmag+\dfrac12\dfrac{\alpha^2}{N}\Ee_\gamma[\sigmag \trace(\Qg^2)]
\end{align*}

Similar to the derivation of~\eqref{eq:drmamlsols}, $\Ee_\gamma[\Ee_{\oO_\gamma}[\rR(\tilde{\btheta}_\gamma(\alpha);\gamma)]]$ is minimized by $\Ee_\gamma[\Ag]^{-1}\Ee_\gamma[\Ag\Thetag]$.

From now on, assume $N\to\infty$.
$\Ag\to(\II-\alpha\Qg)\Qg(\II-\alpha\Qg)=\SSS_\gamma(\alpha)$, so $\Ee_\gamma[\Ag]^{-1}\Ee_\gamma[\Ag\Thetag]\to\mamlsol=\Ee_\gamma[\SSS_\gamma(\alpha)]^{-1}\Ee_\gamma[\SSS_\gamma(\alpha)\Thetag]$.
The expected loss after adaptation of $\mamlsol$ is given by
\begin{align}\label{eq:mamlsolloss}
    &\dfrac12\mamlsol\trans\Ee_\gamma[\SSS_\gamma(\alpha)]\mamlsol-\Ee_\gamma[\SSS_\gamma(\alpha)\Thetag]\trans\mamlsol+\dfrac12\Ee_\gamma[\Thetag\trans \SSS_\gamma(\alpha)\Thetag] \notag \\
    &\quad+\dfrac12\Ee_\gamma[\sigmag] \notag \\
    &=\dfrac12\Ee_\gamma[\Thetag\trans \SSS_\gamma(\alpha)\Thetag]-\dfrac12\Ee_\gamma[\SSS_\gamma(\alpha)\Thetag]\trans\Ee_\gamma[\SSS_\gamma(\alpha)]^{-1}\Ee_\gamma[\SSS_\gamma(\alpha)\Thetag]+\dfrac12\Ee_\gamma[\sigmag]
\end{align}
For $\alpha=0$, \eqref{eq:mamlsolloss} is equal to the expected loss before adaptation of $\drsol$, $\Ee_\gamma[\rR(\drsol;\gamma)]$, i.e. the minimum possible loss before adaptation.
Therefore, to show that for $0<\alpha\leq 1/\beta$, the expected loss after adaptation of $\mamlsol$ is at most $\Ee_\gamma[\rR(\drsol;\gamma)]$, it suffices to show that \eqref{eq:mamlsolloss} is nonincreasing in $\alpha$ on $[0,1/\beta]$.
We do so by computing its derivative with respect to $\alpha$ and showing that it is nonpositive on $[0,1/\beta]$.

Using the chain rule of matrix calculus,
\begin{align*}
    \dfrac{d\eqref{eq:mamlsolloss}}{d\alpha} &= \alpha\Ee_\gamma[\Thetag\trans\Qg^3\Thetag]-\Ee_\gamma[\Thetag\trans\Qg^2\Thetag]-\dfrac12\dfrac{d\Ee_\gamma[\SSS_\gamma(\alpha)\Thetag]}{d\alpha}\trans\Ee_\gamma[\SSS_\gamma(\alpha)]^{-1}\Ee_\gamma[\SSS_\gamma(\alpha)\Thetag] \\
    &\quad-\dfrac12\Ee_\gamma[\SSS_\gamma(\alpha)\Thetag]\trans\dfrac{d\Ee_\gamma[\SSS_\gamma(\alpha)]^{-1}}{d\alpha}\Ee_\gamma[\SSS_\gamma(\alpha)\Thetag] \\
    &\quad-\dfrac12\Ee_\gamma[\SSS_\gamma(\alpha)\Thetag]\trans\Ee_\gamma[\SSS_\gamma(\alpha)]^{-1}\dfrac{d\Ee_\gamma[\SSS_\gamma(\alpha)\Thetag]}{d\alpha} \\
    &=-\Ee_\gamma[\Thetag\trans\Qg(\II-\alpha\Qg)\Qg\Thetag]+\Ee_\gamma[\Qg^2\Thetag-\alpha\Qg^3\Thetag]\trans\Ee_\gamma[\SSS_\gamma(\alpha)]^{-1}\Ee_\gamma[\SSS_\gamma(\alpha)\Thetag] \\
    &\quad-\Ee_\gamma[\SSS_\gamma(\alpha)\Thetag]\trans\Ee_\gamma[\SSS_\gamma(\alpha)]^{-1}\Ee_\gamma[\Qg^2-\alpha\Qg^3]\Ee_\gamma[\SSS_\gamma(\alpha)]^{-1}\Ee_\gamma[\SSS_\gamma(\alpha)\Thetag] \\
    &\quad+\Ee_\gamma[\SSS_\gamma(\alpha)\Thetag]\trans\Ee_\gamma[\SSS_\gamma(\alpha)]^{-1}\Ee_\gamma[\Qg^2\Thetag-\alpha\Qg^3\Thetag] \\
    &=-\Ee_\gamma[\Thetag\trans\Qg(\II-\alpha\Qg)\Qg\Thetag]+\Ee_\gamma[\Qg(\II-\alpha\Qg)\Qg\Thetag]\trans\Ee_\gamma[\SSS_\gamma(\alpha)]^{-1}\Ee_\gamma[\SSS_\gamma(\alpha)\Thetag] \\
    &\quad-\Ee_\gamma[\SSS_\gamma(\alpha)\Thetag]\trans\Ee_\gamma[\SSS_\gamma(\alpha)]^{-1}\Ee_\gamma[\Qg(\II-\alpha\Qg)\Qg]\Ee_\gamma[\SSS_\gamma(\alpha)]^{-1}\Ee_\gamma[\SSS_\gamma(\alpha)\Thetag] \\
    &\quad+\Ee_\gamma[\SSS_\gamma(\alpha)\Thetag]\trans\Ee_\gamma[\SSS_\gamma(\alpha)]^{-1}\Ee_\gamma[\Qg(\II-\alpha\Qg)\Qg\Thetag] \\
    &=-\Ee_\gamma\left[(\Thetag-\Ee_\gamma[\SSS_\gamma(\alpha)]^{-1}\Ee_\gamma[\SSS_\gamma(\alpha)\Thetag])\trans\Qg(\II-\alpha\Qg)\Qg(\Thetag-\Ee_\gamma[\SSS_\gamma(\alpha)]^{-1}\Ee_\gamma[\SSS_\gamma(\alpha)\Thetag])\right]
\end{align*}
which is the negative of an expectation of a quadratic form with inner matrix $\Qg(\II-\alpha\Qg)\Qg$.
When $0<\alpha\leq 1/\beta$, $\Qg(\II-\alpha\Qg)\Qg$ is positive semidefinite for all $\gamma$, and the derivative is nonpositive.

\end{proof}

% From Lemma~\ref{lem:prepostupdatelossfunc}, 
% \begin{align*}
%     \Ee_\gamma[f(\gamma,\drest)] &= \dfrac12\drest\trans\Ee_\gamma[\Qg]\drest-\Ee_\gamma[\Qg\Thetag]\trans\drest+\dfrac12\Ee_\gamma[\Thetag\trans\Qg\Thetag]+\dfrac12\Ee_\gamma[\sigmag] \\
%     \Ee_\gamma[\Ee_{\oO_\gamma}[f(\gamma,\tilde{\hat{\theta}}_{DR,\gamma}(\alpha))]] &= \dfrac12\drest\trans\Ee_\gamma[\Ag]\drest-\Ee_\gamma[\Ag\Thetag]\trans\drest+\dfrac12\Ee_\gamma[\Thetag\trans\Ag\Thetag] \\
%     &\quad+\dfrac12\Ee_\gamma[\sigmag]+\dfrac12\dfrac{\alpha^2}{N}\Ee_\gamma[\sigmag \trace(\Qg^2)]
% \end{align*}

% We rewrite the above to include $\drest-\drsol$.
% \begin{align}\label{eq:drprebound}
%     \Ee_\gamma[f(\gamma,\drest)] &= \dfrac12(\drest-\drsol)\trans\Ee_\gamma[\Qg](\drest-\drsol)-\Ee_\gamma[\Qg\Thetag]\trans\drest \notag \\
%     &\quad+\dfrac12\Ee_\gamma[\Thetag\trans\Qg\Thetag]+\dfrac12\Ee_\gamma[\sigmag]-\dfrac12\theta_{DR}^{*\intercal}\Ee_\gamma[\Qg]\drsol+\theta_{DR}^{*\intercal}\Ee_\gamma[\Qg]\drest \notag \\
%     &= \dfrac12(\drest-\drsol)\trans\Ee_\gamma[\Qg](\drest-\drsol)+\dfrac12\Ee_\gamma[\sigmag] \notag \\
%     &\quad+\dfrac12\Ee_\gamma[\Thetag\trans\Qg\Thetag]-\dfrac12\Ee_\gamma[\Qg\Thetag]\trans\Ee_\gamma[\Qg]^{-1}\Ee_\gamma[\Qg\Thetag] \notag \\
%     &\leq \dfrac12\norm{\Ee_\gamma[\Qg]}\norm{\drest-\drsol}^2+\Ee_\gamma[f(\gamma,\drsol)]
% \end{align}
% where the second equality follows from the expression for $\drsol$ in Proposition~\ref{prop:drmamlsols}.
% Similarly,
% \begin{align}\label{eq:drpostbound}
%     &\Ee_\gamma[\Ee_{\oO_\gamma}[f(\gamma,\tilde{\hat{\theta}}_{DR,\gamma}(\alpha))]] \notag \\
%     &= \dfrac12(\drest-\drsol)\trans\Ee_\gamma[\Ag](\drest-\drsol)-\Ee_\gamma[\Ag\Thetag]\trans(\drest-\drsol) \notag \\
%     &\quad+\dfrac12\Ee_\gamma[\Thetag\trans\Ag\Thetag]+\dfrac12\Ee_\gamma[\sigmag]+\dfrac12\dfrac{\alpha^2}{N}\Ee_\gamma[\sigmag \trace(\Qg^2)] \notag \\
%     &\quad-\dfrac12\theta_{DR}^{*\intercal}\Ee_\gamma[\Ag]\drsol+\theta_{DR}^{*\intercal}\Ee_\gamma[\Ag]\drest-\Ee_\gamma[\Ag\Thetag]\trans\drsol \notag \\
%     &=\dfrac12(\drest-\drsol)\trans\Ee_\gamma[\Ag](\drest-\drsol)-\Ee_\gamma[\Ag\Thetag]\trans(\drest-\drsol) \notag \\
%     &\quad+\dfrac12\Ee_\gamma[\Thetag\trans\Ag\Thetag]+\dfrac12\Ee_\gamma[\sigmag]+\dfrac12\dfrac{\alpha^2}{N}\Ee_\gamma[\sigmag \trace(\Qg^2)] \notag \\
%     &\quad+\theta_{DR}^{*\intercal}\Ee_\gamma[\Ag](\drest-\drsol)+\dfrac12\theta_{DR}^{*\intercal}\Ee_\gamma[\Ag]\drsol-\Ee_\gamma[\Ag\Thetag]\trans\drsol \notag \\
%     &=\dfrac12(\drest-\drsol)\trans\Ee_\gamma[\Ag](\drest-\drsol) \notag \\
%     &\quad+(\Ee_\gamma[\Ag]\drsol-\Ee_\gamma[\Ag\Thetag])\trans(\drest-\drsol)+\Ee_\gamma[\Ee_{\oO_\gamma}[f(\gamma,\tilde{\theta}_{DR,\gamma}^*(\alpha))]] \notag \\
%     \begin{split}
%     &\leq\dfrac12\norm{\Ee_\gamma[\Ag]}\norm{\drest-\drsol}_2^2+\Ee_\gamma[\Ee_{\oO_\gamma}[f(\gamma,\tilde{\theta}_{DR,\gamma}^*(\alpha))]] \\
%     &\quad+\norm{\drsol-\theta_A^*(\alpha)}\norm{\Ee_\gamma[\Ag]}\norm{\drest-\drsol} 
%     \end{split}
% \end{align}

% From Lemma~\ref{lem:prepostupdatelossfunc}, 
% \begin{align*}
%     \Ee_\gamma[f(\gamma,\mamlest)] &= \dfrac12\mamlest\trans\Ee_\gamma[\Qg]\mamlest-\Ee_\gamma[\Qg\Thetag]\trans\mamlest \\
%     &\quad+\dfrac12\Ee_\gamma[\Thetag\trans\Qg\Thetag]+\dfrac12\Ee_\gamma[\sigmag] \\
%     \Ee_\gamma[\Ee_{\oO_\gamma}[f(\gamma,\tilde{\hat{\theta}}_{MAML,\gamma})]] &= \dfrac12\mamlest\trans\Ee_\gamma[\Ag]\mamlest-\Ee_\gamma[\Ag\Thetag]\trans\mamlest \\
%     &\quad+\dfrac12\Ee_\gamma[\Thetag\trans\Ag\Thetag]+\dfrac12\Ee_\gamma[\sigmag]+\dfrac12\dfrac{\alpha^2}{N}\Ee_\gamma[\sigmag \trace(\Qg^2)]
% \end{align*}

% We rewrite the above to include $\mamlest-\mamlsol$.
% \begin{align}\label{eq:mamlprebound}
%     &\Ee_\gamma[f(\gamma,\mamlest)] \notag \\
%     &= \dfrac12(\mamlest-\mamlsol)\trans\Ee_\gamma[\Qg](\mamlest-\mamlsol) \notag \\
%     &\quad-\Ee_\gamma[\Qg\Thetag]\trans(\mamlest-\mamlsol)+\dfrac12\Ee_\gamma[\Thetag\trans\Qg\Thetag]+\dfrac12\Ee_\gamma[\sigmag] \notag \\
%     &\quad-\dfrac12\theta_{MAML}^{*\intercal}\Ee_\gamma[\Qg]\mamlsol+\theta_{MAML}^{*\intercal}\Ee_\gamma[\Qg]\mamlest-\Ee_\gamma[\Qg\Thetag]\trans\mamlsol \notag \\
%     &= \dfrac12(\mamlest-\mamlsol)\trans\Ee_\gamma[\Qg](\mamlest-\mamlsol) \notag \\
%     &\quad-\Ee_\gamma[\Qg\Thetag]\trans(\mamlest-\mamlsol)+\dfrac12\Ee_\gamma[\Thetag\trans\Qg\Thetag]+\dfrac12\Ee_\gamma[\sigmag] \notag \\
%     &\quad+\dfrac12\theta_{MAML}^{*\intercal}\Ee_\gamma[\Qg]\mamlsol+\theta_{MAML}^{*\intercal}\Ee_\gamma[\Qg](\mamlest-\mamlsol) \notag \\
%     &\quad-\Ee_\gamma[\Qg\Thetag]\trans\mamlsol \notag \\
%     \begin{split}
%     &\leq \dfrac12\norm{\Ee_\gamma[\Qg]}\norm{\mamlest-\mamlsol}^2+\Ee_\gamma[f(\gamma,\mamlsol)] \\
%     &\quad+\norm{\mamlsol-\drsol}\norm{\Ee_\gamma[\Qg]}\norm{\mamlest-\mamlsol}
%     \end{split}
% \end{align}
% where the final inequality uses the expression for $\mamlsol$ in Proposition~\ref{prop:drmamlsols}.
% Similarly,
% \begin{align}\label{eq:mamlpostbound}
%     &\Ee_\gamma[\Ee_{\oO_\gamma}[f(\gamma,\tilde{\hat{\theta}}_{MAML,\gamma}(\alpha))]] \notag \\
%     &= \dfrac12(\mamlest-\mamlsol)\trans\Ee_\gamma[\Ag](\mamlest-\mamlsol) \notag \\
%     &\quad-\Ee_\gamma[\Ag\Thetag]\trans(\mamlest-\mamlsol)+\dfrac12\Ee_\gamma[\Thetag\trans\Ag\Thetag]+\dfrac12\Ee_\gamma[\sigmag] \notag \\
%     &\quad+\dfrac12\dfrac{\alpha^2}{N}\Ee_\gamma[\sigmag \trace(\Qg^2)]-\dfrac12\theta_{MAML}^{*\intercal}\Ee_\gamma[\Ag]\mamlsol+\theta_{MAML}^{*\intercal}\Ee_\gamma[\Ag]\mamlest \notag \\
%     &\quad-\Ee_\gamma[\Ag\Thetag]\trans\mamlsol \notag \\
%     &=\dfrac12(\mamlest-\mamlsol)\trans\Ee_\gamma[\Ag](\mamlest-\mamlsol) \notag \\
%     &\quad-\Ee_\gamma[\Ag\Thetag]\trans(\mamlest-\mamlsol)+\dfrac12\Ee_\gamma[\Thetag\trans\Ag\Thetag]+\dfrac12\Ee_\gamma[\sigmag] \notag \\
%     &\quad+\dfrac12\dfrac{\alpha^2}{N}\Ee_\gamma[\sigmag \trace(\Qg^2)]+\theta_{MAML}^{*\intercal}\Ee_\gamma[\Ag](\mamlest-\mamlsol) \notag \\
%     &\quad+\dfrac12\theta_{MAML}^{*\intercal}\Ee_\gamma[\Ag]\mamlsol-\Ee_\gamma[\Ag\Thetag]\trans\mamlsol \notag \\
%     \begin{split}
%     &\leq \dfrac12\norm{\Ee_\gamma[\Ag]}\norm{\mamlest-\mamlsol}^2+\Ee_\gamma[\Ee_{\oO_\gamma}[f(\gamma,\tilde{\theta}_{MAML,\gamma}^*(\alpha))]] \\
%     &\quad+\norm{\mamlsol-\Ee_\gamma[\Ag]^{-1}\Ee_\gamma[\Ag\Thetag]}\norm{\Ee_\gamma[\Ag]}\norm{\mamlest-\mamlsol}
%     \end{split}
% \end{align}

==> Neurips2020 (3)/tex/metarl_details.tex <==
\subsection{Setup}

\paragraph{Environments}
We consider four robotic locomotion and four manipulation environments, all with continuous action spaces.
The robotic locomotion environments, based on MuJoCo~\citep{mujoco} and OpenAI Gym~\citep{gym}, fall into two categories.
\begin{itemize}
    \item Varying reward functions: HalfCheetahRandVel, Walker2DRandVel
    
    The HalfCheetahRandVel environment was introduced in~\citet{maml}.
    The distribution of tasks is a distribution of HalfCheetah robots with different goal velocities, and remains the same for meta-training and meta-testing.
    The Walker2DRandVel environment, defined similarly to HalfCheetahRandVel, is found in the codebase for~\citet{promp}.
    
    \item Varying system dynamics: HopperRandParams, Walker2DRandParams
    
    The HopperRandParams and Walker2DRandParams were introduced in~\citet{promp}.
    For HopperRandParams, the distribution of tasks is a distribution of Hopper robots with different body mass, body inertia, damping, and friction, and remains the same for meta-training and meta-testing.
    The Walker2DRandParams environment is defined similarly.
\end{itemize}

We briefly describe the four manipulation environments from Metaworld; for more details please refer to~\citet{metaworld}.
\begin{itemize}
    \item ML1-Push and ML1-Reach: ML1-Push considers the manipulation task of pushing a puck to a goal position. The distribution of tasks is a collection of initial puck and goal positions, and differs for meta-training and meta-testing. ML1-Reach is defined similarly to ML1-Push but with the manipulation task of reaching a goal position.
    \item ML10 and ML45: For both environments, the meta-training and meta-testing distributions of tasks are collections of manipulation tasks and the corresponding initial object/goal positions. The manipulation tasks in the meta-training versus meta-testing distributions do not overlap; there are $10$ manipulation tasks in the training distribution for ML10, and $45$ for ML45.
\end{itemize}

\paragraph{Algorithms}
We consider four policy gradient algorithms, ProMP~\citep{promp}, which approximately combines MAML and PPO~\citep{ppo}, DRS+PPO, a combination of DRS and PPO, TRPO-MAML~\citep{maml}, and DRS+TRPO, a combination of DRS and TRPO~\citep{trpo}.
For full descriptions of the ProMP and TRPO-MAML algorithms, please refer to the cited papers. We use the implementations in the codebase provided by~\citet{promp}.
To combine DRS and PPO/TRPO, it suffices to take the original PPO/TRPO algorithm and maximize the objective using generated trajectories from a sampled set of tasks instead of a single task.
This follows from the fact that we can approximate an expectation over a distribution of tasks by a Monte Carlo sample of tasks.

\paragraph{Meta-training}
ProMP and TRPO-MAML use the same meta-training procedure~\citep{promp, maml}.
At each iteration, a set of $M$ tasks are sampled from the meta-training distribution of tasks.
For each task, ProMP (TRPO-MAML) generate $L$ episodes under the current policy, computes an adapted policy using policy gradient, and generates $L$ episodes under the adapted policy; all $M\times L$ episodes generated under adapted policies are used to compute its objective.
For each task, DRS+PPO (DRS+TRPO) generate $L$ episodes under the current policy; all $M\times L$ episodes are used to compute its objective.

Each iteration of ProMP (TRPO-MAML) requires twice as many steps from the simulator as DRS+PPO (DRS+TRPO).
Therefore, to ensure that each algorithm utilizes the same amount of data, we run ProMP (TRPO-MAML) for half as many iterations as DRS+PPO (DRS+TRPO).
More specifically, for the robotic locomotion environments, we run ProMP (TRPO-MAML) for $1000$ iterations and DRS+PPO (DRS+TRPO) for $2000$.
For the manipulation environments, we run ProMP (TRPO-MAML) for $10000$ iterations and DRS+PPO (DRS+TRPO) for $20000$.
These go beyond the number of training steps used in~\citet{promp} and~\citet{metaworld}.

\paragraph{Meta-testing}
The meta-testing procedure, described next, are carried out at $21$ checkpoints during meta-training.
We sample $1000$ tasks from the meta-testing distribution of tasks.
For each task and ProMP/DRS+PPO (TRPO-MAML/DRS+TRPO), starting at a meta-trained policy, we repeat the following five times: 1) generate $L$ episodes from the current policy and 2) update the policy with the same policy gradient algorithms used to compute the adapted policies while training ProMP (TRPO-MAML).
We compute the average episodic reward after $t$ policy updates, for $t=0,1,\dots,5$.
These statistics are then compiled over all $1000$ sampled tasks, using the procedure outlined below.

For ProMP and TRPO-MAML, the learning rate used to update the policy is the inner learning rate used to compute the adapted policies during meta-training. For DRS+PPO, it is the learning rate during meta-training (our heuristic), and for DRS+TRPO, it is zero.

\paragraph{Hyperparameters}
To choose the meta-training learning rates, step sizes, and the inner learning rate used to compute the adapted policies, we conduct grid search. 
For the robotic locomotion environments, the learning rate for ProMP and DRS+PPO was chosen from $[0.0001, 0.001, 0.01]$, the step size for TRPO-MAML and DRS+TRPO from $[0.001, 0.01, 0.1]$, and the inner learning rate for ProMP and TRPO-MAML from $[0.01, 0.05, 0.1]$. 
For the manipulation environments, the learning rate for ProMP and DRS+PPO was chosen from $[0.000001, 0.00001, 0.0001, 0.001]$, the step size for TRPO-MAML and DRS+TRPO from $[0.001, 0.01, 0.1]$, and the inner learning rate for ProMP and TRPO-MAML from $[0.00001, 0.0001, 0.001, 0.01]$.
These ranges include the values given in the codebases for~\citet{promp} and~\citet{metaworld}.
The chosen values are given in Table~\ref{tab:lrs}.
%For TRPO-MAML, we use the inner learning rates and step sizes given by~\citet{promp} and personal communication with the authors of~\citet{metaworld}.
%Specifically, for all environments, the step size is set to $0.01$ and the inner learning rate is $0.01$.
%The step size for DRS+TRPO is $0.01$ for all environments.

\begin{table}[ht]
    \centering
    \ra{1.3}
    \begin{tabular}{@{}ccccccc@{}}
    \toprule
    Environment & \multicolumn{2}{c}{ProMP} & DRS+PPO & \multicolumn{2}{c}{TRPO-MAML} & DRS+TRPO \\
    \cmidrule{2-3} \cmidrule{4-4} \cmidrule{5-6} \cmidrule{7-7}
    & LR & Inner LR & LR & Step Size & Inner LR & Step Size \\
    \midrule
    HopperRandParams & 0.001 & 0.01 & 0.001 & 0.1 & 0.01 & 0.1 \\
    Walker2DRandParams & 0.001 & 0.01 & 0.001 & 0.1 & 0.01 & 0.1 \\
    HalfCheetahRandVel & 0.0001 & 0.01 & 0.01 & 0.001 & 0.01 & 0.01 \\
    Walker2DRandVel & 0.001 & 0.01 & 0.001 & 0.1 & 0.01 & 0.01 \\
    ML1-Push & 0.0001 & 0.0001 & 0.0001 & 0.1 & 0.0001 & 0.1 \\
    ML1-Reach & 0.0001 & 0.0001 & 0.0001 & 0.001 & 0.00001 & 0.001 \\
    ML10 & 0.0001 & 0.001 & 0.0001 & 0.01 & 0.001 & 0.001 \\
    ML45 & 0.0001 & 0.00001 & 0.0001 & 0.1 & 0.001 & 0.01 \\
    \bottomrule
    \end{tabular}
    \caption{Learning rates (LR), step sizes, and inner learning rates chosen by grid search.}
    \label{tab:lrs}
\end{table}

For the remaining hyperparameters, we used the values given in~\citet{promp} and~\citet{metaworld}.
We list below several of the main ones:
\begin{itemize}
    \item $M$: $40$ for the robotic locomotion environments, $20$ for the manipulation environments
    \item $L$: $20$ for the robotic locomotion environments, $10$ for the manipulation environments
    \item Episode length: $200$ for the robotic locomotion environments, $150$ for the manipulation environments
    \item Policy architecture: a multi-layer perceptron with two hidden layers of $64$ nodes for the robotic locomotion environments, and $100$ nodes for the manipulation environments.
    \item A linear feature baseline is used to compute the advantage values.
\end{itemize}

\paragraph{Result Compilation}
We run meta-training and meta-testing for all environments and algorithms for five random seeds.
For a fixed environment, algorithm, and checkpoint, let the per seed estimates of the average rewards and their variances to be $\hat{R}_s, \hat{V}_s$, $s=1,\dots,5$, and $R$ to be the corresponding random variable with mean $\mu$ and variance $\sigma^2$.
The estimated mean of $R$, $\hat\mu$, is computed as the average of the $\hat{R}_s$.
Using the formula $\var[R]=\Ee[\var[R\mid s]]+\var[\Ee[R\mid s]]$, $\hat{\sigma}^2$, the estimated variance of $R$, is computed as the sum of 1) the average of the $\hat{V}_s$ and 2) the variance of the $\hat{R}_s$.

To compute the probability that DRS is better than MAML, we use the one sided Welch's t-test. Although the t-test makes the underlying assumption of Gaussianity, it is an acceptable assumption as reporting mean and variance is the common practice. Let the estimated average rewards be $\hat\mu_{drs}$ and $\hat\mu_{maml}$ and their estimated standard deviations be $\hat\sigma_{drs}$ and $\hat\sigma_{maml}$. Since we use five random seeds, we compute the t-value and degree of freedom as 
\begin{equation}
    t = \left(\hat\mu_{drs} - \hat\mu_{maml}\right) / \sqrt{\frac{\hat\sigma_{drs}^2}{5} + \frac{\hat\sigma_{maml}^2}{5}} \quad \text{and} \quad \nu= \frac{\left(\hat\sigma_{drs}^2/5 + \hat\sigma_{maml}^2/5\right)^2}{(\hat\sigma_{drs}^2/5)^2/4 + (\hat\sigma_{maml}^2/5)^2/4}
\end{equation}
We compute the probability of $\mu_{drs}>\mu_{maml}$ as one minus the CDF of a t-distribution with $\nu$ degrees of freedom at $t$.




\subsection{Additional Results}

In this section we present results in a way that is more commonly seen in the meta-RL literature.
We plot the average reward after one policy update at meta-testing as a function of the number of steps at meta-training.
Figures~\ref{fig:pporeward} and~\ref{fig:trporeward} shows the plots for each environment for ProMP \& DRS+PPO and TRPO-MAML \& DRS+TRPO, respectively.

For the first two environments with variations in system dynamics only, seen in Figure~\ref{fig:pporeward}-(a,b) and~\ref{fig:trporeward}-(a,b), DRS is superior to MAML throughout training.
For the next four environments with variations in reward functions only, either 1) DRS and MAML are comparable (Figure~\ref{fig:pporeward}-(d) and~\ref{fig:trporeward}-(e,f)), or 2) while DRS is initially superior, as the amount of training data increases the difference between the two algorithms usually diminishes, and eventually MAML may surpass DRS  (Figure~\ref{fig:pporeward}-(c,e,f) and~\ref{fig:trporeward}-(c)).
In the final two environments with variations in system dynamics and reward functions, the standard errors are generally too large to make a definite statement (see Figure~\ref{fig:pporeward}-(g,h) and~\ref{fig:trporeward}-(h)). 
This suggests that useful inductive biases are more difficult to learn when the system dynamics vary between tasks, a potentially interesting direction for further study.

\begin{figure}
    \centering
    \begin{subfigure}[b]{0.24\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/ppo_hopper_params_reward_update_1.png}
        \caption{HopperRandParams}
        \label{fig:ppohopperparamsreward}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.24\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/ppo_walker_params_reward_update_1.png}
        \caption{Walker2DRandParams}
        \label{fig:ppowalkerparamsreward}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.24\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/ppo_cheetah_goal_reward_update_1.png}
        \caption{HalfCheetahRandVel}
        \label{fig:ppocheetahgoalreward}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.24\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/ppo_walker_goal_reward_update_1.png}
        \caption{Walker2DRandVel}
        \label{fig:ppowalkergoalreward}
    \end{subfigure}
    \\
    \begin{subfigure}[b]{0.24\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/ppo_ml1push_reward_update_1.png}
        \caption{ML1-Push}
        \label{fig:ppoml1pushreward}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.24\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/ppo_ml1reach_reward_update_1.png}
        \caption{ML1-Reach}
        \label{fig:ppoml1reachreward}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.24\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/ppo_ml10_reward_update_1.png}
        \caption{ML10}
        \label{fig:ppoml10reward}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.24\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/ppo_ml45_reward_update_1.png}
        \caption{ML45}
        \label{fig:ppoml45reward}
    \end{subfigure}
    \caption{DRS+PPO vs. ProMP: Average episodic rewards after one update of the policy during evaluation, as a function of the number of steps at meta-training. DRS+PPO is \textcolor{red}{red} and ProMP is \textcolor{blue}{blue}.}
    \label{fig:pporeward}
\end{figure}

\begin{figure}
    \centering
    \begin{subfigure}[b]{0.24\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/trpo_hopper_params_reward_update_1.png}
        \caption{HopperRandParams}
        \label{fig:trpohopperparamsreward}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.24\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/trpo_walker_params_reward_update_1.png}
        \caption{Walker2DRandParams}
        \label{fig:trpowalkerparamsreward}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.24\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/trpo_cheetah_goal_reward_update_1.png}
        \caption{HalfCheetahRandVel}
        \label{fig:trpocheetahgoalreward}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.24\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/trpo_walker_goal_reward_update_1.png}
        \caption{Walker2DRandVel}
        \label{fig:trpowalkergoalreward}
    \end{subfigure}
    \\
    \begin{subfigure}[b]{0.24\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/trpo_ml1push_reward_update_1.png}
        \caption{ML1-Push}
        \label{fig:trpoml1pushreward}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.24\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/trpo_ml1reach_reward_update_1.png}
        \caption{ML1-Reach}
        \label{fig:trpoml1reachreward}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.24\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/trpo_ml10_reward_update_1.png}
        \caption{ML10}
        \label{fig:trpoml10reward}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.24\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/trpo_ml45_reward_update_1.png}
        \caption{ML45}
        \label{fig:trpoml45reward}
    \end{subfigure}
    \caption{DRS+TRPO vs. TRPO-MAML: Average episodic rewards after one update of the policy during evaluation, as a function of the number of steps at meta-training. DRS+TRPO is \textcolor{red}{red} and TRPO-MAML is \textcolor{blue}{blue}.}
    \label{fig:trporeward}
\end{figure}

==> Neurips2020 (3)/tex/metarl_experiments.tex <==
We study the trade-off empirically in meta-reinforcement learning in this section. We compare DRS and MAML on on a wide range of meta-RL benchmarks used in the literature. We consider 1) four robotic locomotion environments introduced by \citet{maml} and \citet{promp}, with varying reward functions (Half Cheetah Rand Vel, Walker2D Rand Vel) or varying system dynamics (Hopper Rand Params, Walker2D Rand Params) and 2) four manipulation environments from MetaWorld~\citep{metaworld} with varying reward functions (ML1-Push, ML1-Reach) or changing manipulation tasks and varying reward functions (ML10, ML45).
\footnote{We do not include ML1-Pick-and-Place because training was unsuccessful for all algorithms of interest.}
All environments utilize the Mujoco simulator~\citep{mujoco}. 

We make two comparisons: 
1) ProMP~\citep{promp}, which combines MAML with PPO~\citep{ppo}, vs. DRS combined with PPO (DRS+PPO)
2) TRPO-MAML~\citep{maml, promp}, which combines MAML with TRPO~\citep{trpo}, vs. DRS combined with TRPO (DRS+TRPO).
Meta-training is controlled such that all algorithms utilize an equal number of steps generated from the simulator for each environment.

During evaluation, we first sample a set of meta-test tasks. For each meta-test task, starting at a trained policy, we repeat the following five times: generate a small number of episodes from the current policy and update the policy using the policy gradient algorithm from the inner optimization of ProMP and TRPO-MAML.
We compute the average episodic reward after $t$ updates, for $t=0,1,\dots,5$.
These statistics are then averaged over all sampled tasks.
We evaluate the policies learned by all algorithms at various checkpoints during meta-training, in total five evaluations with different random seeds. For each checkpoint and test update, we compute the probability of DRS being better than MAML using the one-sided Welch t-test. We plot the filled contour plot of the probabilities with respect to the meta-training checkpoint and number of test updates in Figures~\ref{fig:ppo} and~\ref{fig:trpo}. 
We include details of the experimental protocol, Welch t-test, and additional plots of the reward in Appendix~\ref{sec:metarl_details}.

\begin{figure}[t]
\includegraphics[width=\textwidth]{figures/ppo_v1.pdf}
\vspace{-5mm}
    \caption{DRS+PPO vs. ProMP: Probability that the first method is better than the second.}
\vspace{5mm}
    \label{fig:ppo}
%\end{figure}
%\begin{figure}
\includegraphics[width=\textwidth]{figures/trpo_v1.pdf}
\vspace{-5mm}
    \caption{DRS+TRPO vs. TRPO-MAML: Probability that the first method is better than the second.}
    \vspace{-5mm}
    \label{fig:trpo}
\end{figure}

For the majority of environments, DRS is either better than or comparable to MAML, \emph{(see Figure~\ref{fig:ppo}-(a,b,d,e,f) and Figure~\ref{fig:trpo}-(a,b,d,e,f))}. For two environments, specifically \emph{Half Cheetah Rand Vel} and \emph{ML10} in Figure~\ref{fig:ppo}-(c,g)\&\ref{fig:trpo}-(c,g), MAML outperforms DRS for larger sample sizes and at least one test update. This confirms our thesis as the higher optimization error of MAML requires a larger sample size for successful learning, dominating its trade-off with modeling error for smaller sample sizes. 
Another surprising result is the case of ML45 (in Figure~\ref{fig:ppo}-(h)\&~\ref{fig:trpo}-(h)) where as the sample size increases it alternates between the cases where DRS is better and MAML is better. We conjecture that this is because of the greater variance in meta training arising from the higher diversity in tasks.


%MAML performs better than DRS only for small quantities of meta-training steps in Figure~\ref{fig:ppo}-(a,b,d,g) and Figure~\ref{fig:trpo}. 
%We believe this is largely due to the fact that DRS does not become effective until some fixed training budget as discussed in Section~\ref{sec:dr_sample_complexity} (see the flat part in Figure~\ref{fig:drtradeoff}). Once the DRS is effective, it consistently performs better than MAML. 
%Partially due to the nonconvexity of the deep reinforcement learning objective, the optimization and statistical errors appear to dominate and makes MAML less effective even for rather large numbers of meta-training steps in Figure~\ref{fig:ppo}-(a,b,e) and Figure~\ref{fig:trpo}-(a,b,d). In the cases of Figure~\ref{fig:ppo}-(d,g,h) and Figure~\ref{fig:trpo}-(c,e,f,g,h), MAML is effective for larger numbers of training steps, but DRS performs nearly as well. It is also interesting to note from Figure~\ref{fig:ppo}-(d,g) and Figure~\ref{fig:trpo}-(e,f,h), that MAML is usually more effective in update sizes $1$ and $2$. This is rather expected as ProMP and TRPO-MAML implicitly assume a single inner optimization step in meta-training and suggests that MAML somewhat overfits.



Another interesting observation is that in the majority of environments, MAML fares better when combined with TRPO than when combined with PPO. This validates the importance of optimization as both TRPO and PPO use exactly the same model and are expected to behave similarly from a statistical perspective. We suspect that this behavior is due to the difference in how the trust region is used for optimization. In TRPO-MAML the constraint on the KL divergence between the current policy and updated policy is strictly enforced, while in ProMP it is transformed into a Lagrangian penalty and thus may not actually be satisfied. Satisfaction of the constraint is more helpful for MAML, whose empirical gradients generally have greater variance than those of DRS.

In conclusion, when the sample complexity is high and available sample size budget is low, DRS is the preferred method. MAML is only effective for large data sets, only in some problems. It is important for practitioners to understand the sample complexity of their problems before choosing which method to apply. In the next section, we provide theoretical analysis to clarify this phenomenon. 





\iffalse
We evaluate the policies learned by all algorithms at various points during training.
Figures~\ref{fig:ppo} and~\ref{fig:trpo} plot the average episodic rewards after the policy update during evaluation as a function of the number of steps in the environment seen during training.
For the environments with varying system dynamics, seen in figures~\ref{fig:ppocheetahgoalreward} and ~\ref{fig:ppowalkergoalreward}, DRS+PPO is superior to ProMP throughout training.
However, for the remaining environments with varying reward functions, while DRS+PPO is initially superior, as the amount of training data increases the difference between the two algorithms diminishes, and eventually ProMP surpasses DRS+PPO for HalfCheetahRandVel and ML1-Reach.
This suggests that useful inductive biases are more difficult to learn when the system dynamics vary between tasks, a potentially interesting direction for further study.
\begin{figure}
    \centering
    \begin{subfigure}[b]{0.24\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/ppo_hopper_params_reward_update_1.png}
        \caption{HopperRandParams}
        \label{fig:ppohopperparamsreward}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.24\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/ppo_walker_params_reward_update_1.png}
        \caption{Walker2DRandParams}
        \label{fig:ppowalkerparamsreward}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.24\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/ppo_cheetah_goal_reward_update_1.png}
        \caption{HalfCheetahRandVel}
        \label{fig:ppocheetahgoalreward}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.24\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/ppo_walker_goal_reward_update_1.png}
        \caption{Walker2DRandVel}
        \label{fig:ppowalkergoalreward}
    \end{subfigure}
    \\
    \begin{subfigure}[b]{0.24\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/ppo_ml1push_reward_update_1.png}
        \caption{ML1-Push}
        \label{fig:ppoml1pushreward}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.24\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/ppo_ml1reach_reward_update_1.png}
        \caption{ML1-Reach}
        \label{fig:ppoml1reachreward}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.24\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/ppo_ml10_reward_update_1.png}
        \caption{ML10}
        \label{fig:ppoml10reward}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.24\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/ppo_ml45_reward_update_1.png}
        \caption{ML45}
        \label{fig:ppoml45reward}
    \end{subfigure}
    \caption{DRS+PPO vs. ProMP: Average episodic rewards after one update of the policy during evaluation, as a function of the number of training steps seen. DRS+PPO is red and ProMP is blue.}
    \label{fig:ppo}
\end{figure}
\fi 

==> Neurips2020 (3)/tex/prelim.tex <==
\label{sec:preliminaries}

Arguably, the major bottleneck of applying machine learning to many practical problems is the cost associated with data and/or labeling. While the cost of labeling and data makes supervised learning problems expensive, the high sample complexity of reinforcement learning makes it downright inapplicable for many practical settings. Meta-learning (or in general multi-task learning) is designed to ease the sample complexity of these methods. 
It has had success stories on a wide range of problems including image recognition and reinforcement learning~\citep{metalearningsurvey}.



In the classical risk minimization setting, for a task $\gamma$, the learner solves the problem
\begin{equation}
    \min_{\btheta} \rR(\btheta; \gamma) \triangleq \Ee_{\xi} \left[\hat{\rR}(\btheta,\xi ;\gamma)\right] 
    \label{eq:test_problem}
\end{equation}
where $\rR(\btheta;\gamma)$ is the risk function which the learner can only access via noisy evaluations $\hat{\rR}(\btheta,\xi;\gamma)$. 
Meta-learning, or `learning to learn'~\citep{thrun98}, makes the observation that if the learner has access to a collection of tasks sampled from a distribution $p(\gamma)$, it can utilize an offline meta-training stage to search for shared inductive biases that assist in learning future tasks from $p(\gamma)$.
Under the PAC framework, \citet{baxter00} shows that given sufficiently many tasks and data per task during meta-training, there are guarantees on the generalization of learned biases to novel tasks.

%Since we are interested in meta-learning setting, $\gamma$ is the task-id and the shared risk function enables inductive bias between problem. Meta-learning makes the observation that, if the learner has access to collection of tasks sampled from distribution $p(\gamma)$, it can utilizes an offline meta-learning step to share inductive bias. 

Specifically, consider an optimization algorithm $\texttt{OPT}(\gamma, \btheta_{meta})$ which solves the problem of meta-test task $\gamma$ using the meta solution $\btheta_{meta}$. This meta solution is typically a policy initialization for reinforcement learning or shared features for supervised learning. However, it can be any useful knowledge which can be learned in the meta-training stage. The family of meta-learning methods solve, where in practice $\texttt{OPT}$ is approximated by $\hat{\texttt{OPT}}$ that uses $N$ calls to an oracle \footnote{For example, if $\texttt{OPT}(\gamma,\btheta_{meta})$ is gradient descent on the task risk function $\rR(\btheta; \gamma)$, $\hat{\texttt{OPT}}(\gamma,\btheta_{meta},N)$ would be SGD on the usual empirical risk minimization function~\eqref{eq:erm}.};
\begin{equation}
    \min_{\btheta} \rR^{meta}(\btheta_{meta}) \triangleq \Ee_{\gamma \sim p(\gamma),\xi} \left[ \hat{\rR}(\texttt{OPT}(\gamma, \btheta_{meta}) ,\xi; \gamma) \right]
    \label{eq:meta_population}
\end{equation}

This setting is intuitive and theoretically sound. However, it corresponds to a complicated bilevel optimization problem. Bilevel optimization is a notoriously hard problem and even the case of a well-behaved inner problem (\eg linear program as $\textsc{OPT}$) can be NP-hard \citep{nphard} in the general case. Hence, one can rightfully ask, is it feasible to solve the meta problem in \eqref{eq:meta_population}? This question is rather more important for the case of reinforcement learning as even solving the empirical-risk minimization in \eqref{eq:test_problem} has prohibitively high sample complexity.


Meta-learning proposes to accurately use the structure of the problem by introducing a very costly optimization problem. One obvious question is, \emph{can we trade off modeling accuracy for computational ease?} Unfortunately, there is no general principled approach for controlling this trade-off as it requires understanding domain specific properties of the meta problem. Instead, we focus on the case of meta-information $\btheta_{meta}$ as the initialization of an iterative optimizer for meta-test task $\gamma$, $\btheta_{meta} = \btheta^0_\gamma$ and drop the subscript \emph{meta} as it is clear from the context. This covers many existing algorithms, including MAML~\citep{maml}, which is able to approximate any learning algorithm when combined with deep networks~\citep{finnuniversality}.
For this case of meta-learning the initialization, a simple and direct alternative would be solving the pseudo-meta problem
\begin{equation}
    \min_{\btheta} \rR^{drs}(\btheta) \triangleq \Ee_{\gamma \sim p(\gamma), \xi} \left[ \hat{\rR}(\btheta,\xi; \gamma) \right]  
    \label{eq:dr_population}
\end{equation}
We call this domain randomized search (DRS) since it corresponds to the domain randomization method from \citet{dr} and it does direct search over a distribution of domains (tasks).
\footnote{It has also been referred to as joint training in the literature~\citep{onlinemetalearning}.}

It might not be clear to the reader how DRS solves meta-learning. It is important to reiterate that this is only the case if the meta-learned information is an initialization. However, we believe an approximate form of meta-learning without bilevel structure can be found in other cases with the help of domain knowledge. In this paper, we rigorously prove that DRS is an effective meta-learning algorithm for learning an initialization by showing DRS decreases sample complexity during meta-testing. %Moreover, we also study the modeling and optimization trade-off of DRS and MAML both empirically and theoretically.

These two approaches correspond to the two extremes of the modeling and optimization trade-off. Meta-learning corresponds to an \emph{accurate modeling} and \emph{a computationally harder optimization}, whereas DRS corresponds to a \emph{less accurate modeling} and \emph{computationally easier optimization}. In this paper, we try to understand this trade-off and specifically attempt to answer the following question; \emph{Given a fixed and finite budget for meta-training and meta-testing, which algorithm is more desirable?} In order to answer this question, we provide a collection of theoretical and empirical answers. Taking MAML to be the representative meta-learning algorithm;
\begin{itemize}
    \item We empirically study this trade-off in meta-reinforcement learning (Section~\ref{sec:metarlexp}).
    \item We analyze the sample complexity of DRS and MAML for a general non-convex function, and illustrate the interplay of the modeling error and optimization error (Section~\ref{sec:complexity}).
    \item We theoretically analyze the meta-linear regression case, which is fully tractable, and explicitly characterize the trade-off with simulations that confirm our results (Section~\ref{sec:linreg}).
\end{itemize}
Code to reproduce the experiments can be found at \url{https://github.com/intel-isl/MetaLearningTradeoffs}.

\subsection{Formulation, Background and Summary of Results}

We are interested in a distribution $p(\gamma)$ of problems with risk functions $\rR(\btheta, \gamma)$ for the task ids $\gamma$. Given a specific task, we assume we have access to $2N$ i.i.d. samples from the risk function. This corresponds to sampling data-points and labels for the supervised learning problem, and sampling episodes with their corresponding reward values for reinforcement learning\footnote{Risk can be seen as the chosen loss function for supervised learning and negative of reward for RL.}. Classical empirical risk minimization separately solves for each $\gamma$
\begin{equation}\label{eq:erm}
    \min_{\btheta} \tilde{\rR}(\btheta; \gamma) \triangleq \frac{1}{2N} \sum_{i=1}^{2N} \hat{\rR}(\btheta, \xi_i; \gamma)
\end{equation}
where $\xi_i$ are datapoints for supervised learning and episodes for RL. Empirical risk minimization for MAML can be defined over $M$ meta-training tasks sampled from $p(\gamma)$ as;
\begin{equation}
    \min_{\btheta} \tilde{\rR}^{maml}(\btheta) \triangleq \frac{1}{M} \sum_{j=1}^M  \frac{1}{N} \sum_{i=1}^{N} \hat{\rR}(\hat{\texttt{OPT}}(\gamma_j, \btheta, N) ,\xi_{i,j}; \gamma_j)
    \label{eq:maml_empirical}
\end{equation}
Meta-learning needs samples for both the inner optimization and outer meta problem; usually half of the samples are used for each. Empirical risk minimization for DRS is
\begin{equation}
    \min_{\btheta} \tilde{\rR}^{drs}(\btheta) \triangleq \frac{1}{M} \sum_{i=1}^M \frac{1}{2N} \sum_{i=1}^{2N} \hat{\rR}(\btheta,\xi_{i,j}; \gamma_j)
    \label{eq:empirical_drs_problem}
\end{equation}

Denote the solutions of problems \eqref{eq:meta_population} and \eqref{eq:dr_population} by $\btheta_{maml}^{\star}$ and $\btheta_{drs}^{\star}$, which are the minimum population risk solutions. We call the risk of these solutions $\rR^{drs}(\btheta_{drs}^\star)$ and $\rR^{maml}(\btheta_{maml}^\star)$ the \textbf{modeling error} as they are the best each method can get with the best optimizer and infinite data and computation. However, we only have access to empirical risk in \eqref{eq:maml_empirical} and \eqref{eq:empirical_drs_problem}, as well as a finite computation budget for meta-training, $T^{tr}$. Hence, instead of optimal solutions, we have solutions $\btheta_{maml}^{T^{tr}}$ and $\btheta_{drs}^{T^{tr}}$. We call the difference between these empirical solutions and $\btheta_{maml}^{\star}$ and $\btheta_{drs}^{\star}$ the \textbf{optimization error}.

We expect the optimization error of MAML to be significantly higher as bilevel optimization is much harder. More specifically, for general non-convex risk functions, in order for stochastic gradient descent (SGD) to reach an $\epsilon$-stationary point, DRS needs $\mathcal{O}(\nicefrac{1}{\epsilon^4})$ samples \citep{sgd_convergence} while MAML needs $\mathcal{O}(\nicefrac{1}{\epsilon^6})$~\citep{mamlconvergence}. Moreover, MAML uses half of its samples for the inner optimization; hence, the effective number of samples is reduced resulting in additional optimization error. The optimization error strongly depends on the sample budget ($N$ and $M$) which can be afforded. As more samples will decrease optimization errors for both methods but with different rates. On the other hand, we know MAML has lower modeling error as it explicitly uses the problem geometry. 

The key question is the trade-off of the modeling error versus the optimization error as a function of $N$ and $M$ since it characterizes which algorithm is better for a given problem and budget. We look at this trade-off in two different settings.
\begin{itemize}
    \item \textbf{General Non-Convex Case:} We study this trade-off empirically for meta-reinforcement learning (Section~\ref{sec:metarlexp}) and theoretically for general non-convex risk functions (Section~\ref{sec:complexity}). Our empirical results suggest that this trade-off is rather nuanced and problem dependent. Our theoretical results shed light on these peculiarities and describe the trade-off.
    
    \item \textbf{Meta-linear regression:} (Section~\ref{sec:linreg}). Empirical risk can be minimized analytically, enabling us to directly compare optimization error and modeling error. Results suggest that there are cut-off values for $N$ and $M$ that determine when the different methods are desirable.
\end{itemize}

==> Neurips2020 (3)/tex/related.tex <==
% Recent meta-learning survey: https://arxiv.org/pdf/2004.05439.pdf
% NOTES: meta-learning as searching for an inductive bias

%Simpler is better: https://arxiv.org/pdf/2003.11539.pdf, https://arxiv.org/pdf/2003.04390.pdf, https://arxiv.org/pdf/2003.06957.pdf, https://arxiv.org/pdf/1911.04623.pdf

%Topics to cover:
%\begin{itemize}
    %\item Meta-learning in general
    %\item Universality of gradient(optimization)-based meta-learning
    %\item Learnability results on meta-learning by Baxter
    %\item Analyses of MAML wrt convexity, sample complexity
    %\item Recent counterintuitive work that does not explicitly use the two-stage nature of meta-learning during training
%\end{itemize}

%Meta-learning, or `learning to learn'~\citep{thrun98}, aims to improve an algorithm's learning performance on future tasks by searching for useful inductive biases from training on similar tasks.
%It has had success stories on a wide range of problems including image recognition and reinforcement learning; see~\citet{metalearningsurvey} for a survey of recent algorithms and applications.
%It also has attractive theoretical properties.
%\citet{finnuniversality} prove that gradient-based meta-learning with deep networks can approximate any learning algorithm.
%Under the PAC framework, \citet{baxter00} show that given sufficiently many tasks during training and data per task, there are guarantees on the generalization of learned biases to novel tasks from the same distribution as in training.

%The vast majority of meta-learning algorithms incorporate knowledge about the testing procedure into the training objective.
%For instance, model-agnostic meta-learning (MAML \citep{maml}) explicitly utilizes the fact that gradients are used to update the model for a test task by minimizing the loss after one (or more) gradient update for all training tasks.
%This approach is intuitively appealing, as it accounts for the structure of the meta-learning problem.

Recent work on few-shot image classification has shown that features from learning a deep network classifier on a large training set combined with a simple classifier at meta-testing may outperform many meta-learning algorithms~\citep{simpleshot, chen2020new, tian2020rethinking}; a similar observation has been made for few-shot object detection~\citep{wang2020frustratingly}.
\citet{benchmarkinggeneralization} show that DRS outperforms RL$^2$ \citep{rl2} on simple reinforcement learning environments where tasks correspond to different system dynamics.
Our meta-RL experiments complement these works and theoretical studies partially explain them.
We argue that there is a larger picture to be considered; the trade-off between modeling accuracy and optimization ease depend on characteristics of the dataset, model, and optimization, and should be studied on a case-by-case basis.

Previous theoretical studies of MAML have primarily focused on the meta-training stage.
\citet{onlinemetalearning} prove that the MAML objective is smooth and convex if the task risk functions are smooth and convex and derive the DRS and MAML estimates if those functions are known for linear regression.
\citet{mamlconvergence} characterize the meta-training sample complexity of SGD for MAML in supervised learning; \citet{mamlconvergencerl} provide analogous results for reinforcement learning.
For regression with overparameterized neural networks, \citet{wang2020convergence} show that gradient descent leads to the global optimum of the empirical MAML objective~\eqref{eq:maml_empirical}.
\citet{franceschi2018bilevel} study the meta-learning problem~\eqref{eq:maml_empirical} when $\texttt{OPT}(\gamma, \bm{\btheta})$ is a minimization operator instead of an iterative optimization procedure, proposing an algorithm with convergence guarantees.
\citet{implicitmaml} propose implicit MAML with analysis of its training sample complexity, providing an alternative method to estimate the gradient of the MAML objective; \citet{grazzi2020iteration} compare the quality of the estimate to that of the original MAML algorithm.

As a counterpart to \citet{mamlconvergence} and \citet{mamlconvergencerl}, \citet{wang2020optimality} provides bounds on the meta-testing performance of an $\epsilon$-stationary point of the MAML objective, assuming that the same set of tasks is used for meta-training and meta-testing.
In contrast to these previous works, we analyze the meta-testing performance and overall optimization behavior of MAML when the meta-training and meta-testing tasks are not identical, merely drawn from the same distribution, and compare them to those of DRS.
